Constant-Time Snapshots with Applications to Concurrent Data Structures

We present an approach for efficiently taking snapshots of the state of a collection of CAS objects. Taking a snapshot allows later operations to read the value that each CAS object had at the time the snapshot was taken. Taking a snapshot requires a constant number of steps and returns a handle to the snapshot. Reading a snapshotted value of an individual CAS object using this handle is wait-free, taking time proportional to the number of successful CASes on the object since the snapshot was taken. Our fast, flexible snapshots yield simple, efficient implementations of atomic multi-point queries on concurrent data structures built from CAS objects. For example, in a search tree where child pointers are updated using CAS, once a snapshot is taken, one can atomically search for ranges of keys, find the first key that matches some criteria, or check if a collection of keys are all present, simply by running a standard sequential algorithm on a snapshot of the tree. To evaluate the performance of our approach, we apply it to two search trees, one balanced and one not. Experiments show that the overhead of supporting snapshots is low across a variety of workloads. Moreover, in almost all cases, range queries on the trees built from our snapshots perform as well as or better than state-of-the-art concurrent data structures that support atomic range queries.

==> conclusion.tex <==
\section{Discussion and Conclusion}

\Eric{For space, I suggest cutting this section.  We really already say all this in the intro.}

In this paper, we show a simple technique for allowing arbitrary computable linearizable queries on a large class of concurrent data structures. 
This is achieved by introducing versioning for each \CAS\ object, and associating all of these objects with a single \snapshot\ object that saves the current sate of all objects at once when accessed. This produces a handle that allows lazily reading a snapshot of the data structure at the time that the handle was produced. 

We show that using such a snapshot handle, we can implement efficient queries for data structures that are \emph{directly linearizable}, i.e., have an abstraction function from the concurrent to the abstract state. Many concurrent data structures in the literature are directly linearizable, and we give examples of how to build efficient queries for a few of them, as well as a technique for finding such queries that is widely applicable. We can always bound the time complexity of query operations in terms of their step complexity when run in isolation, plus a small contention factor. Furthermore, the time complexity of other operations remains unchanged.
%
We also show how to optimize the versioned construction to avoid potential cache misses when possible. 

When using multiversioning, it is crucial to be able to garbage collect outdated versions that will never be accessed, since otherwise the data structure's space usage can grow alarmingly fast. In Appendix~\ref{sec:gc}, we show that classic epoch based memory reclamation can be used safely on our versioned data structure implementation.

We believe that techniques introduced in this paper are practical and widely applicable for concurrent data structures to support linearizable wait-free queries of their global state.

==> doubly-linked-list.tex <==

\subsection{Doubly Linked List}

\subsubsection{Interface}

\begin{itemize}
 \item
\end{itemize}

\subsubsection{Algorithm}

\label{sec:dll}

Each version lists is implemented as a doubly linked list under the hood. This doubly linked list needs to support 4 operations: \var{peakHead}, \var{pushHead(key, val)} (key guaranteed to be non-decreasing), \var{remove(n)} (\var{n} points to a node), \var{search(key)}. Algorithm \ref{fig:dll-alg} shows how these operations can be implemented.

\begin{figure*}
  \begin{lstlisting}[linewidth=.99\columnwidth, numbers=left]
class Node {
  int key; Value val;
  Node* next, prev;
  bool mark;
  Node(Key k, Value v, Node* n) { // constructor
    val = v; key = k; mark = false;
    next = n; prev = nullptr; }

class DoublyLinkedList {
  Node* head;
  DoublyLinkedList() { // constructor
    head = new Node(-inf, @$\bot$@, NULL); }
  Value peak_head() { return head->val; }
  
  // precondition: keys are guaranteed to be non-decreasing
  void push_head(Key k, Value v) {
    Node* oldN = head;
    Node* newN = new Node(k, v, oldN);
    while(!CAS(&head, oldN, newN)) {
      oldN = head;
      newN->next = oldN; }
    oldN->prev = newN;
    // it's ok to set oldN->prev here because oldN cannot be deleted until 
    // after this operation completes. }

  // Precondition: n is not at the head of the list and n's replacemant has
  // been completely inserted. This means n->next and n->prev are both not null.
  void remove(Node* n) {
    n->mark = true;
    Node* next = n->next; Node* prev = n->prev;
    Node* nextPrev, prevNext;
  restart:
    whie(true) {
      next, prev = findUnmarked(next, prev);
      nextPrev = next->prev;
      prevNext = prev->next;
      if((next, prev) == findUnmarked(next, prev)) break; }
    if(!CAS(&next->prev, nextPrev, prev)) goto restart;
    if(!CAS(&prev->next, prevNext, next)) goto restart; }

  // Returns a pair of nodes (next, prev). At the linearization point  of this 
  // operation, next and prev are unmarked, but everything in between is marked.
  (Node*, Node*) findUnmarked(Node* n, Node* p) {
  restart:
    while(n->marked) n = n->next;
    while(p->marked) p = p->prev;
    if(n->marked) goto restart;
    return (n, p); }

  Value search(int k) {
    Node* n = head;
    while(k < n->key) {
      n = n->next; }
    return n->val; } }
  \end{lstlisting}
\caption{Doubly linked list implementation}
\label{fig:dll-alg}
\end{figure*}

\subsubsection{Correctness and Complexity}

\begin{itemize}
  \item Only marked nodes are shortcutted out.
  \item Once a \var{remove(n)} operation completes, \var{n} will be shortcutted out.
  \item Once a node is shortcutted out, it cannot appear back in the list. (Due to correctness of the \var{findUnmarked} operation).
  \item I think remove operations take $O(P)$ amortized time.
  \begin{itemize}
    \item Each process will only visit a node in the linked list a constant number of times (during \var{findUnmarked}). This is because once a node is visited, it will be spliced out by the process's \var{remove} operation and thus it won't be visited by this process again.
  \end{itemize}
\end{itemize}

==> experiments.tex <==
\section{Experimental Evaluation}
\label{sec:exp}

\input{experiment-figures}

To unserstand the practical effectiveness of our snapshotting algorithm we have implemented it in both Java and C++ and have applied it to two existing lock-free binary search tree data structures.  Our code uses the optimization discussed in Section~\ref{sec:opt} to avoid indirection, as well as the optimization to avoid repeated timestamps.  The user interface supplies a version field to add to an object to make it ``versionable'', and a vCAS object that can store a pointer to a versionable object.  Modifying a concurrent algorithm involves adding the version fields, making shared mutable locations into vCAS objects, and ensuring the versionable objects are only recorded once.

The goals of our experiments are the following.    We firstly want to understand the overhead of 



% We experimentally evaluate our \snaptransform{} by focusing on its application to
To experimentally evaluate our \snaptransform{}, we apply it to an unbalanced lock-free binary search tree, \bst{} \cite{EFRB10}, and a balanced lock-free binary search tree, \chromatic{} \cite{BER14}.
%, yielding \vbst{} and \vchromatic{} respectively. 
We call the resulting snapshottable data structures \vbst{} and \vchromatic{} respectively.
% \Naama{Here, I would already introduce the names vcas\chromatic{} and vcas\bst{}.}
We measure the overhead of our transformation and compare with several state-of-the-art range queryable data structures.
We implemented our data structures in both Java and C++ and plan to make our code publicly available when the paper is published.
% Our experiments were run in Java.

% \paragraph{Statistics for Intro}
%   - When compare to state-of-the-art balanced concurrent trees, we are faster by X on some workloads, and competitive with them on all other workloads.
%   - The overhead our transformation adds to the original tree is also low, between a and b across a wide range of workloads
%   - Our result suggests that we can focus on designing fast concurrent data structures without worrying about scans.

\myparagraph{Our Java Implementation.}
We started with Java implementations of \bst{} and \chromatic{} obtained from~\cite{trevorimpl}, and applied our snapshot transformation from Section \ref{sec:query} with the optimizations of Section~\ref{sec:opt}.
% The first optimization implies that we only need to use \VCAS{} objects for the left and right pointers of each node and the second optimization allows us to avoid a layer of indirection.
A precondition for one of the optimizations is that the original data structure is recorded-once. 
This condition is naturally satisfied by \chromatic{}, but not by \bst{} because its delete operation performs a pointer swing (via CAS) where the new value is a node that already exists in the data structure.
To avoid this, we slightly modify the delete operation so that it makes a copy of the node and swings the pointer to this new copy instead.
This requires adding some additional marking and helping steps to preserve correctness and lock-freedom.
Once the recorded-once property is satisfied, our \snaptransform{} was very easy to apply.

We implement range queries for both our trees by simply taking a snapshot and running a sequential algorithm as described in Section \ref{sec:query}.
For \vchromatic{}
% our transformed \chromatic{} \Naama{I would use `vcas\chromatic{}' instead of `our transformed \chromatic'}
, we implement and measure the overhead of three additional query operations: \succr{}, \findif{}, and \multisearch{}, to show the performance of \vchromatic{} on more complex queries. With our transformation, these queries are all atomic. 
The \succr($k$, $c$) query takes a key $k$ and returns the first $c$ key-value pairs in the dictionary with key greater than $k$.
The \findif{} operation is part of the C++ standard library~\cite{findif} and it returns the first key-value pair satisfying a given predicate in a given key range.
The \multisearch{} operation takes in a list of keys and returns the values associated with those keys or \nullv{} if the key is not in the data structure.
\Yihan{Since we are giving the parameters of \succr{}, should we also explain the parameters in \findif{} and \multisearch{}}
\Hao{We should probably move these definitions to the preliminaries. I believe these definitions are also repeated elsewhere in the paper.}
% It's easy to extend our implementations with addition query operations by just taking a snapshot and writting a sequential algorithm.

To allow for automatic garbage collection, we use a simplified form of an epoch based memory reclamation to eventually disconnect nodes from the version lists.
The idea is to retire version list next pointers instead of retiring nodes, where ``freeing'' a next pointer simply involves setting it to \nullv{}.
% Only operations that access next pointers in the version list need to announce the current epoch.
% Therefore, \findop{}, \insertop{}, and \deleteop{}, don't announce any epochs.
% We also apply an optimization to shorten the version chain length by compressing if there are two nodes in a row with the same timestamp.
% More specifically, before and after each \vcas{}, we check if the node at the head of the version list has the same timestamp as the next node.
% If it does, we shortcut out the next node.
% This works because we only need to keep the most recent version for each timestamp to support linearizable snapshots.

% Even with Java's automatic garbage collection, our Vcas algorithm prevents nodes from being collected because they are always reachable via the version lists.
% Therefore, we use a simplified version of epoch based collection to eventually set next pointers to null in the version list.

Previous work has shown that range query performance critically depends on batching keys in nodes \cite{FPR19, WSJ18, BBBGHKS17, BA12}.
We use the same batching technique from \pbst{} \cite{FPR19} and \lfca{} \cite{WSJ18}, which stores up to $m$ key-value pairs in each leaf.
Leaves are immutable; inserting a key into a leaf requires making a new copy of the leaf.
The keys in each leaf are stored in sorted order (for binary search).
Inserting into a full leaf involves spliting it into two leaves, each with half the keys.
A full description of this technique can be found in \cite{FPR19}.
We applied batching with $m=64$ to \vbst{} and \vchromatic{} and call the resulting implementations \vbbst{}, \vbchromatic{}.
To measure overhead, we also applied it to the two original data structures, yielding \bbst{}, and \bchromatic{}.
% as well as the two original data structures and call the resulting implementations \vbbst{}, \vbchromatic{}, \bbst{}, and \bchromatic{}.
% We implemented a version of \vbst{} and \vchromatic{} with $m=64$ and call the resulting algorithms \vbbst{} and \vbchromatic{}.
% We use $m=64$ in all our java implementations.
% For consistency, we use $m=64$ for our implementations as well as \lfca{} and \pbst{}.
We found that this batching optimization also improves \findop{}, \insertop{}, and \deleteop{} performance for large trees as it decreases the height of the tree as well as the number of child pointers stored.

% After applying these changes, we call the resulting snapshottable trees \vbbst{} and \vbchromatic{} respectively. 
% \Naama{The names on the plots are a bit different.} \Hao{fixed}
% To measure overhead, we applied the same batching technique to the original Java implementations of \bst{} and \chromatic{}, yielding \bbst{} and \bchromatic{}.

\myparagraph{Our C++ Implementation.}
% We also implemented a C++ version of our transformation to compare with recent work by Arbel-Raviv and Brown \cite{AB18}.
% They present a transformation for
% our transformation in C++ to compare with recent work by Arbel-Raviv and Brown.
% The purpose of our C++ experiments is to compare with recent work by A and B on harnessing epoch based collection for snapshots \cite{AB18}.
% \Hao{edit below}
% We also implemented our approach in C++ to compare with a recent technique by Arbel-Raviv and Brown~\cite{AB18}.
We started with the C++ implementation of a lock-free unbalanced BST obtained from \cite{AB18}, which naturally satisfies our recorded-once property.
We applied our \snaptransform{} with the optimizations in Section \ref{sec:opt} and used our snapshot operation to add atomic range queries to the original BST.
We did not apply the batching optimization since it was also not used by the C++ implementation we compare against \cite{AB18}.
% We did not the batching optimization since it was not used by our C++ competitor \cite{AB18}.
% , but we did not the batching optimization since it was not used by Arbel-Raviv and Brown.
We were able to directly use the epoch based garbage collector that came with original program without any modification.
The code from \cite{AB18} was very well structured, so applying our transformation took less than 150 lines of code.
We call the resulting implementation \vbst{}.

\myparagraph{Competition}
We compare with several state-of-the-art dictionary data structures supporting range queries: \kiwi{}~\cite{BBBGHKS17}, \lfca{}~\cite{WSJ18}, \pbst{}~\cite{FPR19}, \kst{}~\cite{BA12}, \snaptree{}~\cite{BCCO10}, and \epochtree{}~\cite{AB18}.
Code for these data structures were provided by their respective authors.
Arbel-Raviv and Brown\cite{AB18} presented several transformations for adding range queries to concurrent data structures, which they implement in C++. 
We use \epochtree{} to refer to their most efficient range queryable, lock-free BST.
% Their most efficient range queryable, lock-free BST is called \epochtree{}, which is what we compare to.
\epochtree{} and \vbst{} add range queries to the same initial BST.
% \Naama{Shorter alternative to the rest of this paragraph: Their most efficient range queriable BST is called \epochtree, which is what we compare to. \epochtree{} and \vbst{} use the same initial BST.}
% The range queriable BST that results from applying Arbel-Raviv and Brown's lock-free transformation to their lock-free BST is referred to as \epochtree{}.
% \epochtree{} is what we call the range queriable BST that results from applying their lock-free transformation to their lock-free BST.
% We use the lock-free version of their transformation because they show it outperforms their lock-based one.
% \epochtree{} and \vbst{} use the same initial BST.

% The data structures we compare with
All the other data structures we compare with are written in Java and
% Other than \epochtree{}, the data structures we compare with are written in Java.
% All the data structure implement a dictionary ADT with \findop{}, \insertop{}, \deleteop{}, and \rangeop{}.
% Furthermore, all these data structures are lock-free except \snaptree{} which uses fine-grained locking.
they are all lock-free except \snaptree{} which uses fine-grained locking.
We classify \kiwi{}, \snaptree{}, \chromatic{}, \vchromatic{} as \emph{balanced} data structures because they guarantee logarithmic search time in the abscence of contention.
For the $k$-ary tree (\kst{}) we used $k = 64$ which was shown to perform well across a variety of workloads \cite{BA12}.
To be consistent with \vbbst{} and \vbchromatic{}, we use batch size 64 for \lfca{} and \pbst{} as well. This batch size has been shown to yield good range query performance \cite{FPR19, WSJ18}.
% We used default parameter settings for KIWI with the exception of MAX\_THREADS.
% We found that setting MAX\_THREADS to $\max(32, \# of threads in experiment)$ improved their performance for lower threads counts.

% PNB-BST doesn't do memory management. \Hao{Maybe not important to mention.}

% We use batch size 64 for KST, PNB-BST, LFCA, VcasBST, and VcasChromaticTree for consistency.
% This is the default batch size for LFCA and the recommended batch size for KST.


\myparagraph{Methodology.}
Our experiments were run on a 72-core Dell R930 with
4 x Intel(R) Xeon(R) E7-8867 v4 (18 cores, 2.4GHz and 45MB L3 cache),
and 1Tbyte memory.  Each core is 2-way hyperthreaded giving 144
hyperthreads. We use
\texttt{numactl -i all} in all experiments, evenly spreading the
memory pages across the processors in a round-robin fashion.
Turbo-boost was disabled.

The machine runs Ubuntu 16.04.6 LTS.
C++ code was compiled with g++ version 9.2.1 and compiler flag \texttt{-O3}.
Jemalloc was used for scalable memory allocation.
For the Java experiments, OpenJDK 11.0.5 was used with flags \texttt{-server}, \texttt{-Xms300G} and \texttt{-Xmx300G}.
The latter two flag reduce interference from Java's GC.
For our Java experiments, we performed 10 runs of 5 seconds each;
the first 5 are used to warm up the JVM and we report the average of the last 5.
In C++, we performed 5 runs of 5 seconds each and report the average.
% Our C++ experiments did not require any warm up runs.
In both C++ and Java, we saw very little variance across the 5 runs.
% Performance was very stable across runs and variance was low in almost all our experiments.
% in 95\% the experiments, standard deviation was below x\%.

\myparagraph{Workload Overview.}
In our workloads, we vary four key parameters: data structure size, operation mix, size of range queries, and number of threads.
% We run experiments on data structures prefilled up to 100K keys and 100M keys.
In most of our experiments, we begin by prefilling a data structure with either 100K or 100M keys and then perform a mix of operations.
An operation mix is represented by four values, $\mathit{ins}$, $\mathit{del}$, $\mathit{find}$, $\mathit{rq}$, which represent the probability for each thread to execute an \insertop{}, \deleteop{}, \findop{}, or \rangeop{}, respectively.
In addition, the parameter $\mathit{rqsize}$ specifies the size of each range query.
Given a key range $r$, keys for each operation are drawn uniformly at random from $[1, r]$.
\Yihan{What is the key range of the initial tree? Is it $100K$ for tree size $100K$?}
% (or $[1, r - rqsize]$ in the case of \rangeop{}).
Key ranges are chosen so that the initial data structure size is maintained.
% initial data structure size is maintained throughout the experiment.
For example, if the initial size is 100K and the workload consists of 30\% inserts and 20\% deletes, we would choose $r = 166K$. 
% We use 100K and 100M for the initial size of our data structures.
\Yihan{Does this $rqsize$ corresponds to the ``size of range queries'' parameter, and $r$ is something different (correspond to all query types)? }

In workloads with uniform random keys, unbalanced BSTs are balanced in expectation, so we also run a workload where keys are inserted in sorted order.
This kind of workload often appears in practice and it is useful for testing the balanced trees.

\Yihan{Generally I feel like the setting could be shortened, but it looks like we are not short of space any way. If we need more space we could do so.}
% Workloads with uniform random keys are ideal for unbalanced BSTs because it makes them balanced in expectation.
% T

\myparagraph{Scalability.}
Figures \ref{fig:exp}a-\ref{fig:exp}f show scalability (in Java) under a variety of operation mixes.
% We used $\{1,36,72,140\}$ for number of threads.
In Figures \ref{fig:exp}c and \ref{fig:exp}f, even though range queries are only performed 1\% of the time, they still occupy a significant fraction of the execution time.
For these experiments, we used thread counts 1, 36, 72, and 140.

In general, our balanced and unbalanced trees perform about the same and scale well across all workloads.
Snaptree is competitive with our trees in the absences of range queries, but it has no scalability when range queries are present due to its lazy copy on write mechanism.
LFCA outperforms our trees in Figure \ref{fig:exp}b, but it is consistently slower in the 100M-key experiments (Figures \ref{fig:exp}d-f).

\Yihan{could also say something like: using 140 threads, in most tested cases, the fastest implementation is one of our two implementations, and our two implementations are almost always among the top three. Also none of the other implementations is consistently faster than our implementation. Overall \chromatic{} performs very well. I saw part of the discussion are now in the conclusion paragraph. Maybe adding a paragraph about overall performance or discuss more details in conclusion?}

% - KIWI doesn't scale because each chunk has to store a cache line padded announcement array and get operations scan a global announcement array on every operation
%   - KIWI scales poorly because each lookup has to scan announcement array of size MAX\_THREADS. Puts don't always scan this array, which sometimes gives then faster performance than lookups. each chunk of 1024 keys has to have an array of size MAX\_THREADS*PADDING for announcement, which uses a lot of space.

\myparagraph{Varying range query size.}
In Figures \ref{fig:exp}g and \ref{fig:exp}h, we show the effect of range query size on update and range query performance.
We used $\{8, 64, 256, 1K, 8K, 64K\}$ for the range query sizes.
These experiments (run in Java) have 36 dedicated range query threads and 36 dedicated update threads.
Each update thread performs 50\% inserts and 50\% deletes on a data structure initialized to 100K keys.
To better understand the cost of updates and range queries, we plot the throughput of each operation separately.
A C++ version of the same experiment is shown in Figures \ref{fig:exp}j and \ref{fig:exp}k.

In Figure \ref{fig:exp}g, \bpbst{} has almost no update throughput when $rqsize$ is 1024 or less.
This is because their update operations are forced to abort and restart whenever a new range query begins, and thus decreasing range query size lowers update throughput.
% and because range queries are more frequent when $rqsize$ is small.
\kst{} performs decently in most workloads except when each range query covers a significant fraction of the key range.
For example in Figure \ref{fig:exp}h, their range query throughput drops below 100 operations per second for range queries of size $8K$ and $64K$.
This is because their range query performs a double collect of the desired range and is forced to restart if it see an update in that range.

Data structures that increment a global timestamp with every range query become bottlenecked by this increment when range queries are frequent.
This applies to our data structure as well as \bpbst{}, \kiwi{}, and \epochtree{}.
Consequently, range queries of size 8 are 3x faster on LFCA than on our trees.
However, \lfca{} avoids using a global timestamp by having update operations help ongoing range query operations.
This helping becomes more frequent and more costly when the range query size is large.
For range queries of size 64K (about a third of the key range), the update throughput of our trees is 4x faster than \lfca{}.
% Also, for range queries of size 1K or larger, the global timestamp is no longer a bottleneck and our range query throughput is as fast as \lfca{}.

Figure \ref{fig:exp}k shows that range queries on \vbst{} are 4.7-6.3x faster than \epochtree{}.
To understand why, we measured the number of nodes visited by range queries on \epochtree{} and \vbst{} and found that \epochtree{} visit 1.5 to 5.5 times more nodes.
This is because a range query on \epochtree{} has to visit three nodes in the retired list for each \deleteop{} it is concurrent with.

% In Figures \ref{fig:exp}j and \ref{fig:exp}k \unsafebst{} represents... with unsafe range queries which sequentially scans the desired range.
% Interestingly, when the global timestamp is not a bottleneck, our atomic range queries are just as fast as unsafe range queries on \unsafebst{}.
% We profiled our code and found that while we execute significantly more instructions and branches, we incur the same number of cache misses as the unsafe version.

 % - Worst case interaction between puts and range queries is when all puts happen in a range of 10K keys and all range queries access this range. This maximizes the chance they will have to traverse version chains. I'm guessing this would affect LFCA and KIWI more than ours.

\myparagraph{Sorted workload.}
In Figure \ref{fig:exp}i, we test the performance of the Java data structures under a sorted workload.
In this experiment, we insert a list of sorted numbers into an initially empty data structure by splitting the array into chunks of size 1024 and placing the chunks on a global work queue; when a thread runs out of work to do, it grabs a new chunk from the head of the work queue.
Throughput numbers for this experiment were less stable so we ran 20 trials and took the average of the last 10 trials.

All unbalanced trees overlap at the bottom of Figure \ref{fig:exp}i.
LFCA is a slight exception because it performs well on 1 thread, but quickly joins the other unbalanced trees at 36 threads.
This is because LFCA is structured an unbalanced tree where each leaf stores a balanced, functional treap.
The unbalanced portion of LFCA grows and shrinks according to the amount of contention.
When there is only a single thread, all keys are stored in a single functional treap so LFCA is balanced.
However on 72 and 140 threads, the unbalanced portion becomes much larger.
We measured the number of nodes traversed in each insert attempt and it was over 2000 on average for both thread counts.

\myparagraph{Overhead of our transformation.}
In Figure \ref{fig:exp}o, we compare our Java implementations of \vbbst{} and \vbchromatic{} with the original data structures, \bbst{} and \bchromatic{}.
The numbers in Figure \ref{fig:exp}o are normalized to the throughput numbers of \bbst{} and \bchromatic{} to make the overheads easier to read.
On 140 threads, the overhead of our transformation is low, ranging between 2.7\% and 9.1\% depending on the workload.
This overhead includes the time for epoch based memory management and the overhead of using \vcas{} and \vrd{}.
For \vbbst{}, it also includes the extra marking we added to make deletion satisfy the recorded-once property.

We also measured the overhead of our multi-point queries such as \rangeop{}, \succr{}, \findif{}, and \multisearch{}.
To do so, we compared the throughput from \vbchromatic{} with the throughput of \emph{non-atomic} multi-point queries on the original \bchromatic{}.
Results are shown in Figure \ref{fig:complex}.
% In Figure \ref{fig:complex}, we show the overhead of \emph{atomic} queries on \vbchromatic{} when compared to \emph{non-atomic} queries on \bchromatic{}.
Non-atomic queries are implemented using sequential algorithms and thus are not linearizable.
For example, non-atomic \multisearch($keys$) simply calls \findop{} for each key in $keys$.
These queries provide a good estimate of the maximum performance we can hope for.

% In Figure \ref{fig:complex}, throughput numbers are normalized to the throughput of non-atomic queries in a workload with no updates.
The numbers in the x-axis represent the size of the query. For example ``successors 128'' returns the next 128 keys starting from a particular key, and ``successors'' simply returns the next key.
% the first 128 successors of a particular key and ``successors'' simply returns one succesor.
``Findif 128'' returns the first key that is a multiple of 128 and ``multisearch 4'' atomically search for a list of 4 keys.
For finding one successor, we are 36.8-41.4\% slower than non-atomic and this is again due to the counter bottleneck.
All other queries are large enough to not encounter this bottleneck, and they are between 2.9\% and 12.8\% slower than their non-atomic counterparts.
Having concurrent updates slows down both the atomic and non-atomic queries by about the same amount.
% This holds even when there are 36 concurrent update threads.
% Overheads of our transformation:
%     - For finding one successor, we are 40\% slower than unsafe. This is again due to the counter bottleneck.
%     - For finding the next 128 successors starting from a key, we have almost no overhead.
%     - Similarly for the other complex queries.
%     - For multisearch, this means that searching for 4 keys atomically is almost as cheap as calling lookup 4 times.
%   - Complex queries:
%     - Implementing these queries simply involved implementing a sequential algorithm
%     - Adding these queries to LFCA and KIWI would be more complicated
%     - These queries could also have been implemented for PBST just as easily
%       - Our persistent BST and PBST support the same set of query operations and the performance would be similar modulo the effect we already talked about
%       - The PBST paper is specific to one data structure and our approach is more general.

\Yihan{It looks like we didn't discuss the difference between having and not having updates?}
\Hao{Added a short discussion of this.}

\myparagraph{Conclusion.}
Overall, our transformation only adds a small amount of overhead (about 3\% to 40\%) to the original data structure and our general transformation performed well compared to existing special purpose data structures.
% \vbst{} has a tradeoff with \lfca{} where it is slower when range query size is small and faster when range query size is large.
In particular, \vchromatic{} had the best overall performance among all the range queryable data structures we evaluated.
\Yihan{Why just the best balanced? It looks like the best over all.} \Hao{I changed it to best overall.}
% Many of these data structures were specifically designed whereas \vbst{} and \vchromatic{} use our general technique.
% Many of the data structures we compared with were specially designed
The main bottleneck in our approach is the global timestamp and it would be interesting to look for efficient ways to circumvent this.


==> gc.tex <==

% Optimization: if there are two nodes in a row with the same timestamp, then you can remove the previous one right away.

\section{Memory Reclamation}
\label{sec:gc}
For memory reclamation, we use Epoch Based Memory Reclamation (EBMR)~\cite{fraser2004practical}. 
EBMR splits an execution 
into epochs by utilizing a global epoch counter \var{EC} (with initial value $1$). 
It supports the operations \beginop\ and \retire.
A process $p$ that invokes an operation $op$ calls \beginop\ to read \var{EC}
and announces the value read.
EBMR maintains a \emph{limbo list} of objects for each epoch.
Objects that are {\em retired}
(e.g., Nodes that are deleted from the data structure) are stored
in the limbo list of the current epoch,
until it is ensured that no process holds a pointer to these objects.
When all processes have announced  they have seen an epoch number that is at least $r$, the limbo list associated
with epoch $r-2$ is collected.  
In this way, EBMR maintains only the limbo lists of the last three epochs. 

This scheme can be applied out of the box in both the indirect (unoptimized)
and direct (optimized) version of our \approach\. We assume that the original concurrent data structure $D$
uses EBMR, and a process invokes \retire{} on a Node $n$ right after the code instructions that 
renters $n$ unreachable. In an execution $\alpha$ of $D$, a Node $n$ is {\em unreachable} 
if it cannot be reached by following pointers in other Nodes 
starting from any entry point of the data structure (otherwise, it is {\em reachable}). 

When using \VerCAS{}, we also invoke \retire{} on the old VNode
after every successful \vcas\ (so that VNodes are also retired). 
Furthermore, we call \retire\ on the head of the version list when the Node containing 
the \vCAS{} object is retired. In this way, we retain the same space bounds that are guaranteed by EBMR.

Note that when \retire\ is called on a Node $n$ in an execution $\alpha$ of $D_{\ell}$,
$n$ may still be reachable through the version list of some \vCAS{} object. 
%Thus, it is not obvious that using the EBMR scheme as is is correct.  
However, we prove that it is safe to deallocate (to free) $n$ by proving 
that no operation will ever traverse as far as $n$ into the version list of the \vCAS\ object.
We say that it is {\em safe} to deallocate an object in an execution
if no process evers refers to this object at some later point in the execution.

\begin{theorem}
Consider a concurrent implementation $D$ of a data structure that uses EBMR for memory reclamation,
and let $D_{\ell}$ be the concurrent implementation we get from $D$ using Construction~\ref{con:sololin}
(and the technique for memory reclamation described above).
	In every execution $\alpha$ of $D_{\ell}$, whenever a Node is deallocated, it is safe to do so.
%If a Node $n$ is deemed safe to be deallocated by the EBMR scheme in the original data structure $D$, 
%then $n$ is also safe to be deallocated in the data structure $D_\ell$ implemented from $D$ using Construction~\ref{con:sololin}.
\end{theorem}

\begin{proof}
Consider any Node $n$ which is deallocated in $\alpha$, and let $r$ be the value of the epoch counter \var{EC} when the deallocation occurs. 
By the way EBMR works, it must be that $r > 2$, and $n$ resides in the limbo list of epoch $r-2$. 
Therefore, $n$ must have been deleted from the data structure during epoch $r - 2$,
i.e., the head of the version list of $n$'s \vCAS\ object has been updated to point from $n$ to another \vnode\ $n'$ during epoch $r-2$. 
Recall that the timestamp of $n'$ is greater than or equal to that of $n$.

Assume that $n$ remains reachable (after its deletion) through the \var{nextv} pointers  of the version list of some \vCAS\ object $O$.
Recall that it is only queries that could access the version list of an object, 
and they may do so only by calling \readss{}. Let $op$ be such a query and let 
\readss($ts$) be any invocation of $op$ that accesses the version list of $O$.
Recall that timestamp $ts$ was acquired when \readss($ts$) invoked \takess{} at the beginning of its execution.
Recall also that \readss($ts$) traverses the version list of the \vCAS\ object starting
from the most recent version (with the largest timestamp among all versions in $O$'s version list) until it reaches the first version 
whose timestamp is smaller than or equal to $ts$. 
%Older versions will never be accessed by \readss{$h$}.

To reach epoch $r$, all processes must have announced epoch $r -1$. 
In particular, this means that no process is still executing 
a query operation that started before epoch $r -1$. 
Thus, all timestamps being used by queries at the point that $n$ is deleted, 
must have been produced after the beginning of epoch $r -1$. 
Therefore, the timestamps they use are greater than or equal to that of $n'$ in the version list of $O$, 
and therefore no \readss{} operation will attempt to access $n$ after its deallocation (they will
stop when reaching $n'$).
Thus, deallocating $n$ is safe.
\end{proof}

%
%\begin{itemize}
%  \item Snapshot and query operations don't need to call \retire{}
%  \item All operations call \var{begin\_op} at the very beginning
%  \item \retire{} and \var{begin\_op} are implemented exactly like in Epoch Based Memory Reclamation
%  \item The space bounds we get are exactly the same as those guaranteed by Epoch Based Memory Management.
%  \item Once a Node is deemed safe to free by Epoch Based Memory Reclamation, it is still techically reachable from the data structure by following version pointers. 
%  However, we can safely free it no operation will ever visit it. 
%  This is because no operation (including snapshot and query operatons) visit Nodes that were retired before the start of the operation.
%\end{itemize}




==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}

We have implemented our snapshotting approach in both Java and C++, on top of three existing implementations (see details below).  Our code uses the optimizations discussed in Section~\ref{sec:opt} to avoid indirection or repeated timestamps.
To apply our \transformation{} on top of an original implementation, our code adds a \snapshot{} object, makes an object \emph{versionable} by adding a \op{version} field to it, and
%uses \vcas{} objects to store original shared mutable pointers to versionable objects.
replaces the original shared mutable pointers to versionable objects by \vcas{} objects.
For employing the optimization to avoid indirection, one should also ensure the versionable objects are only recorded once. For each implementation, we use one global \snapshot{} object.


\Naama{Possible reorganization of the Java and C++ paragraphs (we can then also give a title to the GC paragraph):
	
We applied our \transformation{} to the two BST structures
described in Section~\ref{sec:query}; \bst{} and \chromatic{}, as well as a lock-free unbalanced BST from \cite{AB18}. The first two were implemented in Java, starting from the Concurrent Data Structures Library (CDSL)~\cite{trevorimpl}. The third was implemented in C++. The authors of \cite{AB18} presented several transformations for adding range queries to concurrent data structures. Their most efficient version is called \epochtree{}.

\myparagraph{Batching.}
Previous work has shown that the performance of concurrent BSTs is improved by batching keys
in nodes~\cite{FPR19, WSJ18, BBBGHKS17, BA12}.  We therefore applied the same batching technique
from \pbst{}~\cite{FPR19} and \lfca{}~\cite{WSJ18} to CDSL, storing up to 64 key-value pairs in each leaf.
A full description of this technique can be found in \cite{FPR19}.
Our experiments indicate that batching improves performance both on the original versions and our snapshotted versions.
We did not apply batching since it was also not used by the C++ implementation we compare against \cite{AB18}.

\myparagraph{Recorded-Once.}
The recorded-once requirement is satisfied by \chromatic{} and \epochtree, so the \transformation{} was simply as described above.
However, the \bst{} does not satisfy it; the delete operation performs a pointer swing (via \cas{}) where the new value is a node that already exists in the data structure.
To avoid this, our implementation makes a copy of the node
and swings the pointer to this new copy instead.  This requires some extra marking
and helping steps to preserve correctness and lock-freedom.
Then the modifications were as described above.

For all data structures, we implemented four different \complex{} queries as shown in Table \ref{tab:complexqueries}.
All these queries simply traverse the snapshot of the tree visiting what is needed.
They are all atomic working on a snapshot.
}

%old version
%We have implemented our snapshotting approach  in both Java and C++.
%Our code uses the optimization discussed in Section~\ref{sec:opt}
%to avoid indirection, as well as the optimization to avoid repeated timestamps.
%Our library interface supplies a version field to add to an object to make
%it ``versionable'', and a vCAS object that can store a pointer to a versionable object.
%Modifying a concurrent algorithm involves adding the version fields to objects
%that need multiple versions, making shared mutable pointers \y{to objects} vCAS objects,
%and ensuring any versionable object is only recorded once into a vCAS object.

%We also support objects that are recorded more than once, albeit with a level of indirection.
% We note that although versioned objects must be ``recorded once'' in our interface, the interface remains fully general, albeit possibly with a level of indirection.  In particular the user can define a versioned "copy object" that simply contains one immutable field, which is to the object $A$ they are trying to persist.  To write $A$ to a new location, they can create a new copy object, point it to $A$, and CAS it into the new location.  This satisfies the recorded-once restriction since the copy object is new.  It, however, requires reading $A$ through the copy object, and hence the level of indirection.

%Using our snapshot library, we implemented the two BST structures
%described in Section~\ref{sec:query}.
In Java, we applied our \transformation{} to the two BST structures
described in Section~\ref{sec:query}.  We started with \bst{} and \chromatic{}
obtained from the Concurrent Data Structures Library (CDSL)~\cite{trevorimpl}.
Previous work has shown that the performance of concurrent BSTs is improved by batching keys
in nodes~\cite{FPR19, WSJ18, BBBGHKS17, BA12}.  We therefore applied the same batching technique
from \pbst{}~\cite{FPR19} and \lfca{}~\cite{WSJ18} to CDSL, storing up to 64 key-value pairs in each leaf.  %Leaves are immutable; inserting a key into a leaf requires making a new copy of the leaf.  The keys in each leaf are stored in sorted order (for binary search).  Inserting into a full leaf involves spliting it into two leaves, each with half the keys.
A full description of this technique can be found in \cite{FPR19}.
Our experiments indicate that batching improves performance both on the original versions and our snapshotted versions.
%\here{Y: Unclear: Are you referring to both algorithms or to one of them? If you refer to both, use plural; otherwise specify to which one you are referring to.}
%\Yihan{Looks like it works for more than one implementations, so I changed to plural.}
%For adding snapshots,
The recorded-once requirement is satisfied by \chromatic{}, so the \transformation{} was simply as described above.
%However, the \bst{}'s delete operation performs a pointer swing (via \cas{}) where the new value is a node
%that already exists in the data structure, and hence is recorded more than once.
However, the \bst{} does not satisfy it; the delete operation performs a pointer swing (via \cas{}) where the new value is a node that already exists in the data structure.
%To avoid this, we slightly modified the delete operation so that it makes a copy of the node
%and swings the pointer to this new copy instead.  This required adding some additional marking
%and helping steps to preserve correctness and lock-freedom.
To avoid this,  we modified their algorithm to make a copy of the node
and swing the pointer to this new copy instead.  This requires some extra marking
and helping steps to preserve correctness and lock-freedom.
It was then transformed to allow for snapshots as described above.
For both tree data structures, we implemented four different \complex{} queries as shown in Table \ref{tab:complexqueries}.
All these queries simply traverse the snapshot of the tree visiting what is needed.
They are all atomic working on a snapshot.
%None of this was rocket science, but in the interest of full disclosure modifying the \bst{}'s delete operation did require understanding the data structure.

\begin{table*}
  \centering \small
  \begin{tabular}{lll}
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  \bf Query & \bf Definition & \bf Parameters in Figure \ref{fig:complex}\\
  \hline
  \rangeop{}$(s,e)$: & All keys in range $[s,e]$ & \texttt{RQ256}: $e=s+256$\\
  \succr{}$(k,c)$ & The first $c$ key-values with key greater than $k$ & \succr{}: $c=1$, or \succr\texttt{128}: $c=128$\\
  %$c=1$ (\succr{}) or $c=128$ (\succr\texttt{128})\\
  \findif{}$(s,e,p)$~\cite{findif}:&The first key-value pair in range $[s,e)$&\findif\texttt{128}: $p(k)=(k~\mathit{mod}~128~\mathit{is}~0)$ \\ %decides if $k$ is a multiply of 128\\
  \multisearch{}$(L)$:& For a list of keys in $L$, return their values (\nullv{} if not found)&\multisearch\texttt{4}: $|L|=4$\\
  \hline
\end{tabular}
  \caption{The \complex{} queries and their parameters we use in experiments. \vspace{-.1in}}\label{tab:complexqueries}
\end{table*}

%We implemented four different \complex{} queries: \rangeop{}, \succr{}, \findif{}, and \multisearch{}.
%A \op{range}$(s,e)$ query returns all keys in the ordered dictionary that belong in the range $[s,e]$.
%The \succr$(k,c)$ query takes a key $k$ and returns the first $c$ key-value pairs in the dictionary with key greater than $k$.
%The \findif{}$(s,e,p)$ query is part of the C++ standard library~\cite{findif}
%and it returns the first key-value pair in the range $(s,e)$
%%\here{Y: Is this range closed or open? I used a closed range above for \op{range}.}
%satisfying the predicate $p$ (a function).
%The \multisearch{}$(L)$ query takes a list of keys $L$ and returns the values associated with those keys,
%or \nullv{} if the key is not in the data structure.
%All these queries simply traverse the snapshot of the tree visiting what is needed.
%They are all atomic working on a snapshot. %since the snapshot is atomic.

In C++, we started with the implementation of a lock-free unbalanced BST~\cite{AB18}, which also satisfies our recorded-once property. We applied the modifications described above. %, which took a couple hours.
%(we thank the authors for a clean and well structured implementation)\Guy{is this right}.
On top of the same data structure, Arbel-Raviv and Brown~\cite{AB18} presented several transformations for adding range queries to concurrent data structures. Their most efficient version is called \epochtree{}.
%\epochtree{} and \vbst{} add range queries to the same initial BST.
We did not apply batching since it was also not used by the C++ implementation we compare against~\cite{AB18}.
%We were able to directly use the epoch-based garbage collector that came with original program without any modification.

To support garbage collection we added a \op{release} operation to the \snapshot{} object, which notifies the garbage collector that the process no longer needs its snapshot.
The \takess{} releases the previous snapshot so a process can only access one snapshot at a time.
In our Java implementation we use an epoch-based memory reclamation \cite{fraser2004practical} to disconnect nodes from the version lists when no longer needed.
%\here{Y: Provide citation for epoch-based memory reclamation.} % The idea is to set the next pointer to \nullv{} if there is no longer any process pointing to an older version as determined by the \op{release}s.
The Java garbage collector will then collect the old versions. % since there will no longer be any pointers to them.
For C++, we directly use the epoch based garbage collector in the implementation in~\cite{AB18} (see below).

In the experiments we refer to the non-snapshotted Java implementations as \bbst{}, and \bchromatic{}, and our modified snapshotted versions as \vbbst{}, and \vbchromatic{}.  For C++ we refer to the implementation in \cite{AB18} as \epochtree{}, and our modified snapshotted version as \vbst{}.  %\Guy{what about original version?}
We plan to make the implementation publicly available via GitHub.




==> intro.tex <==
% !TEX root =  main.tex

\section{Introduction}
\label{sec:intro}

The ability to take snapshots of a data structure %at points in time 
is useful for a variety of applications.  In a concurrent setting,
snapshots allow for arbitrary (computable) read-only queries on a data structure even when it is being updated concurrently.
% In principle the updates
% need not wait for the read-only queries, and the read-only queries need
% not wait on the updates, while all properly linearizing.
Snapshots can
also be used to %travel back in time to 
view what the data
structure contained at some point in the past.  In database systems,
snapshots can be used to recover state when the database is
corrupted---perhaps by the inclusion of malicious or invalid
updates.  Due to its usefulness, snapshotting has been used widely in
a variety of settings, including database
systems~\cite{Reed78,BG83,papadimitriou1984concurrency,Postgres12,SQL13,neumann2015fast,Wu17},
persistent sequential data
structures~\cite{sarnak1986planar,driscoll1989making,DST91}, and
concurrent data
structures~\cite{perelman2010maintaining,Attiya11,Kumar14,FPR19,BBSW19}.
Snapshots are often used for multi-versioning, or persistence,
and we sometimes refer to snapshots as versions.
%, and sometimes refer to taking a snapshot as persisting.


% There have been two main approaches to support snapshots.  The first
% is to use functional data
% structures~\cite{Myers83,Myers84,KT96,Okasaki98}.  In this approach
% existing data is never mutated, and updates are made by copying the
% path to where a change is made.  A snapshot, or version, is simply a
% pointer to the structure at the given point in time.  The second is to use version
% lists~\cite{Reed78,BG83,sarnak1986planar,driscoll1989making,DST91}.
% In this approach every low-level object, e.g. memory location, keeps a
% list of its versions sorted by version number, an an update of a
% low-level object adds a new version with the current time stamp.

In this paper we describe a transformation to convert any %algorithm or
shared data structure built from CAS objects and immutable data to
support lazy snapshots of the current state.  The methodology supports
standard reads and CAS on the \emph{current state} of each object.
It then supplies the ability to take lazy snapshots of the state of the
system---i.e., the value of all CAS objects at the current
point in the history.  We call this a lazy snapshot because
the operation does not explicitly return
the values of all CAS objects.
Instead, it returns a
\emph{handle} that can then be used to read the value of any CAS object
at the time the snapshot was taken.  
%This allows traversing a data structure in the state it was
%at the snapshot.  
Our transformation has the following properties:

\begin{itemize}
\item
Taking a snapshot of the current state (and getting the associated handle) takes constant time.

\item CAS and read operations on the current state take constant
  time.  This implies that any asymptotic bounds on time for the
  original data structure are preserved.  Therefore, lock-freedom and
  wait-freedom are preserved, and operations are never delayed by other
  processes reading a snapshot.

\item Reading an old value of a CAS object using a handle takes time proportional
  to the number of successful CASes linearized on the object since the snapshot that produced the handle was taken.
  All reads are wait free.

\item The transformation uses single-word read and CAS.  It
  does, however, require an unbounded timestamp counter.
\end{itemize}

\Eric{Note: I updated ``timestamp'' to ``handle'' when talking about the spec of snapshots
(for consistency with later sections) but since the next
sentence mentions that we use timestamps as the handle in our implementation,
I think it is okay to then use ``timestamp'' when talking about our particular implementation
of \takess, etc.}

Our transformation is based on using integer timestamps as handles, and keeping a version
list~\cite{Reed78,BG83,sarnak1986planar,driscoll1989making,DST91}
for each CAS object.    A version list consists of one node per update
(successful CAS) on the object, each consisting of the value of the
update and the timestamp at the time of the update.  The list is
sorted by timestamp, most recent first.  Taking a snapshot
involves reading the current timestamp, and then ensuring it is
incremented.  An important aspect of the implementation is
the method by which a \CAS\ installs a timestamp in the newest node in the version list.
The idea is to CAS a new node to the front of the version list, but
to temporarily leave its timestamp as \emph{to-be-decided} (TBD).
Once the node has been added to the list, its timestamp is then set (also using a \CAS) to the current value of the counter.
Importantly, any concurrent read or \CAS\ operation that sees this node has to help set its timestamp.
The \CAS\ operation is linearized when the timestamp of the node it added is set.
We note that predetermining the node's timestamp
before adding it to the version list does not work because the timestamp
can be out of date by the time the node gets added.
% \Hao{Predetermining the timestamp is common in lots of prior work \cite{trevor brown, FPR19} and it is one of the main reasons why they are lock-free and we are wait-free constant time.}
% \Eric{Hao's sentence might be misleading:  I wouldn't say that this is the main reason updates are not wait-free in \cite{FPR19}; BST updates can be blocked by other updates even without versioning.  However, it is true that the predetermined timestamps do cause a lot of issues that require handshaking, more coordination between processes.}
% \Hao{My previous comment was poorly worded. The idea I wanted to capture was that using our technique, BST updates can only abort and restart due to other BST updates. In contrast, if you predetermine timestamps, then BST updates can be aborted by snapshots/queries.}
Reading a CAS object at timestamp $v$
involves traversing the version list until a timestamp equal or
less than $v$ is found, and returning the corresponding value.

\myparagraph{Queries on Linearizable Objects.}
For a linearizable implementation of an abstract object we would like
to add support a broad set of queries that use the snapshot and linearize
properly.  This is possible as long as the queries can be
implemented by examining the low-level state (combined state of the
CAS objects) at the current time.  For certain
reasonable data structures, this might not be possible since
%a linearization point in the past can be decided in the future.
we may not know whether an update that is in progress has been linearized yet.
For example, whether the update should be linearized earlier could depend on what happens
later in the execution.
If, in addition to being linearizable, there is an
\emph{abstraction function} $f$ from the low-level state to an
abstract state, then the abstract state is uniquely defined by each
low-level snapshot\footnote{Herlihy and
  Wing~\cite{herlihy1990linearizability} considered abstraction
  functions and showed that to allow all linearizable implementations
  requires a relation instead.}.  The \emph{abstract state} can be
defined by the data structure designer (e.g., sets of integer keys for
an integer set), and state transitions must line up with the
corresponding linearization point (e.g., \textsc{s.insert}$(1)$ would
transition the abstract state from $\{2\}$ to state $\{1,2\}$ at the linearization point
of the \textsc{insert}).  Having an abstraction function is similar
in some ways to strong linearizability~\cite{GHW11}, but neither of these conditions implies the other
(see Appendix~\ref{sec:strong}).  Many, if not most, implementations of
concurrent data structures allow an abstraction function to the
desired state, at least if the linearization points are selected
appropriately.

Although having an abstraction function ensures we can answer any
(computable) query on the abstract state, it does not by itself say
anything about performance.  To get a handle on performance, and
equally importantly to simplify writing queries, we suggest a
methodology based on defining an intermediate \emph{query state},
built out of \emph{query objects}.  The query state is more abstract
than the low-level state but less abstract than the abstract state.
Query objects are read-only.  For example, consider a concurrent set
implemented with binary search trees (BST) augmented with various tags
and flags to support synchronization among the updates 
(as in \cite{EFRB10} or \cite{NM14}, for example).  Here the
query state can be the BST, and the query objects are the nodes of
the tree supporting operations such as left, right, and value, but no
update and with no tags and flags.  The designer of the data structure then
needs to define a function $g$ from low-level state to query state.
To prove correctness with respect to the abstract state they also have
to supply a function $h$ from query state to abstract state, and prove
that $h$ composed with $g$ is equivalent to the abstraction function
$f$.
The definition of $h$ can usually rely on ``textbook''
mappings---e.g., from a BST to an ordered set.  In most cases the
function $g$ is also simple, just involving a projection that ignores
some extra data such as the tags and flags.  In practice, at least in the examples we
consider showing $g \circ h = f$ is not very difficult. Figure \ref{fig:functions} shows
an example about the abstract state, query state and low-level state.

The data structure can also assign a time cost to operations on the query
state.  On a BST, accessing a child pointer would, for example,
have time proportional to the number of concurrent updates to that
child.    We refer to this as the \emph{write contention}.
%\Hao{Maybe separate the cost of taking the snapshot from the cost of the quiescent query.}
%\Guy{Not as clean as I would like it to be since updates are on the low-level pointer.}

Based on these ideas we consider a variety of concurrent data
structures and show that many structures can be implemented to support
a very broad set of queries using our techniques.  In particular we
consider the following data structures.  Here by time we mean
the time not including any write-contention.
\Eric{I'm not sure what preceding sentence means}

\begin{figure}
  \centering
  \begin{minipage}{0.78\columnwidth}
    \includegraphics[width=1\columnwidth]{example2.pdf}
  \end{minipage}
  \begin{minipage}{0.2\columnwidth}
  \caption{An example about abstract state, query state and low-level state.}\label{fig:functions}
  \end{minipage}
\end{figure}

\Hao{It would be nice to give time bounds}

\begin{itemize}
\item MS Concurrent queues~\cite{MS96}.  Here the query state is a linked
  list ordered by the position in the queue from the head, with a pointer to the
  head and tail.  Hence a query can access any element in the queue.
\item
Harris's linked lists~\cite{Harris01}.   Here the query state is an ordered linked list
with a pointer to the head.   A query can find any element.
\item Ellen et al.'s non-blocking binary search trees~\cite{EFRB10}.
  Here the query state is a binary search tree.  This can support
  a broad set of queries such as range queries, next query (next larger key), first
  query, or queries that find all keys that satisfy some predicate.
\item
Skip lists \Note{(probably too much?....leave for journal version?)}
\end{itemize}
In all cases the query time is proportional to the number of distinct
pointers traversed plus the sum of the write contention on each
pointer.   For example, finding the first key in a BST will take time
proportional to depth of that key, plus the number of successful concurrent
updates along the path.
% \Hao{I'm guessing links refer to pointers that are not in the version list?}

\myparagraph{Optimizations.}
We go on to consider some optimizations to our approach.  We first
consider techniques for avoiding creating version lists.  There are
two cases we consider.  The first is if a CAS object is only
successfully written into once, and the abstract state only depends on
the value after the write.  In this case, there is only ever one
version so there is no need for a list of versions.  For example, the
key in a tree node is typically only written to once when the node is created.  
Another more subtle example is that the next pointers in
MS queues~\cite{MS96} need not be multiversioned since they are only
written to once, and if the linearization point is made to be the
pointer swing on the tail, the state does not depend on the next
pointer until after the write.  The second, and likely more important
case in which version lists can be avoided is for information that is
stored in the low-level state that is not needed for the function $g$
that maps to the query state.  In many data structures this includes
various sorts of marks and tags and flags that are used to synchronize
and ensure linearizability of the updates, but need not be examined
for queries.  For example, in Ellen et al.'s binary search
trees~\cite{EFRB10}, the only \CAS\ objects that need to be persisted
are the child pointers in the tree structure itself.  The pointers to
operation descriptors that are used to facilitate helping need not be persisted.

A second optimization is to avoid the level of indirection implied by
version lists.  In particular when using version lists as described,
reading a value from a \CAS\ object requires first reading the location
of the head of the version list, and then reading the value contained
in the head.  This could cause two cache misses for every read.  
\Eric{Omit next sentence?}
We could place the first link of the version list in the CAS object
itself, but this would require a three-word wide \cas\ to atomically
update the version, value and next pointer.  
We say that an object is
\emph{written once}, if a pointer to it is the new value of a
successful \cas\ at most once (note that is distinct from being written
into once, as discussed above).  We show that if objects of a given type
are always written once, then a \CAS\ object that holds pointers to that
type can avoid indirection.  Instead of using a version list, the
timestamp and pointer to the next older version can be placed directly on the
objects.  Note that initializing a \CAS\ object, or even multiple 
\CAS\ objects, to contain a written-once object does not count as a write.
Most tree-like structures can be implemented with this restriction and
completely avoiding the level of indirection.  We give an example for
the trees of Ellen et. al.~\cite{EFRB10}.  
\Eric{I find this next bit confusing.}
We also show that the full
generality of arbitrary \CAS\ objects can be built from just
written-once objects.  This simulation itself requires a level of
indirection, but it indicates that in the general case the restriction
is no worse than than the fully general case in terms of pointer
indirections, but often can be better.

\myparagraph{Garbage Collection.}
Finally we consider the problem of garbage collection.  A legitimate
worry when keeping snapshots is the extra memory needed to keep
multiple versions.  We describe a GC technique based on epochs that collects
the same data-structure objects as an epoch-based collector
on the non-snapshotted version.  It will require extra memory for the
version links, but this is bounded by the number of successful updates
to CAS object since the oldest query (\Guy{is this right.   Perhaps it
  should be ``since the beginning of an epoch'' since an epoch can
  contain multiple versions.}).     Furthermore the time bounds are no
worse than epoch based collection.



==> optimizations.tex <==
\section{Optimizations}
\label{sec:opt}

Consider a concurrent implementation $D$ that is directly linearizable and implements an
abstract data type $A$. Let $F$ be the abstraction function from $\hat{Q}_D$ to $Q_A$. 
Suppose we add a set of $k$ query operations to $A$ to get the ADT $A'$,
and let $R_i$ be the result function of the $i$-th such query, $1 \leq i \leq k$ (see Section~\ref{sec:queries}).
Let $D'$ be the directly linearizable implementation of $A'$ using versioned \CAS\ objects (as described in Section~\ref{sec:snap-query}).

\subsection{Reducing  the Number of \vCAS{} Objects}

The first optimization aims at examining cases where the creation of version lists can be avoided. 
This will be accomplished by leaving some of the \CAS\ objects of $D$ {\em unversioned}, 
i.e., by not replacing them  with \vcas\ objects.
We call a \CAS\ object $O$ {\em safe} if in every execution $\alpha$ of $D$,
no \CAS\ instruction that is performed on $O$ in $\alpha$ fixes the linearization point of any operation. 
We say that a \CAS\ instruction {\em fixes} the linearization point of an operation in $\alpha$
if in the annotation $\alpha'$ provided for $\alpha$ by the abstraction function, 
the configuration that results from the execution of the \CAS\ is followed by a linearization point.
A \CAS\ object that is not safe is {\em unsafe}.
\Youla{This has to be further formalized/corrected based on the corrections/changes we will perform 
in Section 5.}

We call $OptD'_1$ the implementation that results when we replace every unsafe \CAS\ object used in $D$ with a \vcas\ object. 
Note that $Opt'_1$ leaves safe \CAS\ objects unversioned. 

To perform a query operation of $A'$ whose result function is $R_i$, 
a process first reads the value of the counter into a local variable \var{ts}
and then performs a \compinc($ts$) on the counter (in a way similar to what happens
in $D'$). Then, the process performs \vrd($ts$) on every versioned \CAS\ object
and a simple \rd\ operation on every \CAS\ object to get a view $S$ of the shared memory. 
It then returns $R_i(F(S))$.

\begin{theorem}
\label{thm:opt1}
$OptD'_1$ is a directly linearizable implementation of $A'$.
\end{theorem}

\begin{proof}
... yet to be written. It will be in the style of the proof of Theorem 19.
\end{proof}


\myparagraph{{\bf Examples}} The \var{key} fields of Nodes both in \MSQ\ and \NBBST,
as well as update fields of Nodes in \NBBST\ (on which flagging and marking is performed)
are safe \CAS\ objects. 
So, we do not have to replace them with \vcas\ objects when we go from 
$D$ to $OptD'_1$. Also, if for \MSQ, we use the second linearization scheme
described in Section~\ref{sec:examples}, then 
the \var{next} fields of pointers are also safe, so we do not have
to replace them with \vcas\ objects. 
%
Apparently, applying the optimization described above significantly
reduces the number of \vcas\ objects that we use in $OptD'_1$ 
in comparison to those we use in $D'$.



\subsection{Avoiding Indirection}

\Youla{record versus struct?}

For applying the second optimization, we focus on \vcas\ objects
that store pointers to other records, e.g., to Nodes
in the data structure implemented by $D$. A Node is usually implemented 
as a record which has a set of fields, some of which are
immutable and the others are \CAS{} objects, with those of them
that are unsafe containing pointers to other Nodes. 
Recall that this pattern is followed
in both algorithms, \MSQ\ and \NBBST\ (Section~\ref{sec:examples}).
In the rest of this section, 
we focus on \vcas\ objects whose values are pointers to other Nodes. 
The initial value of such a \vCAS\ object may be NULL or a pointer to some other Node. \Hao{We don't allow initial value to be NULL anymore.}

We assume that in $D$ (and therefore also in $D'$), there are one or more entry points (handles) 
to the data structure, and that every operation accesses Nodes of the data structure
through these entry points. 

\begin{definition}
Consider any execution $\alpha$ of $D'$. We say that 
a Node is {\em recorded-once} in $\alpha$, 
	if a pointer to it, is the \var{newV} parameter of a \emph{successful} \vcas\ (that could be applied on any \vCAS\ object 
allocated in $\alpha$) at most once. 
\end{definition}

We say that the implementation $D'$ is {\em recorded-once}
%(the implementations obtained from $D$ as described in Section~\ref{}), 
if for every execution of $D'$, 
every Node used in the execution is recorded-once.
Note that even if $D'$ writes NULL into a \vcas\ object repeatedly, it can be easily transformed to a recorded-once
implementation as follows: whenever a NULL value is to be used as the \var{newV} parameter of a \vcas\ on $O$, 
a new dummy node of type NULL is created (with its \var{nextv} field being equal to NULL) 
and the \vcas\ is called with a pointer to this node as its \var{newV} parameter.
We assume that $D'$ follows this technique to handle NULL pointers.

The optimization can be applied if $D'$ is a recorded-once implementation
and works as follows. 
For each unsafe \vCAS\ object $O$ (storing a pointer to a Node) in $D'$, 
instead of creating a new VNode to store the version pointer 
and the timestamp, the optimization stores this information directly in the Node pointed to by $O$ %that gets pointed to 
(thus avoiding the level of indirection introduced by VNodes).
This requires expanding each Node object with two extra fields.
Figure~\ref{fig:vcas-direct-alg} shows the new version of a Node record 
and provides pseudo-code for \vrsnap, \vrd, and \vcas\  
after the optimization has been applied.
We call the optimized implementation of a \vCAS\ object, \OptVCAS,
and the optimized implementations of \vrsnap, \vrd, and \vcas, \ovrsnap, \ovrd, and \ovcas, respectively.
We refer to the algorithm provided in Section~\ref{sec:vcas}, as \VerCAS.
\Youla{The last sentence should be deleted and the name \VerCAS\ should be introduced
in Section~\ref{sec:vcas}.}
We denote by $OptD'_2$ the resulting implementation. 
(Note that we do not apply the optimization to \vCAS\ objects implementing the entry points.)
\Hao{Is it because the entry points are immutable?}


\myparagraph{{\bf Correctness of OptVerCAS}}
We now focus on a single \vCAS\ object $O$ and show that \OptVCAS\ is linearizable when it is applied on $O$. 
To do so, we need the following definition. 
%Let $\delta$ be any execution of \OptVCAS\ on $O$. 
\begin{definition}
We say that $O$ is a {\em distinct-values \vCAS\ object} if 
each value written into $O$ is distinct. %and
%\item the initial value of $O$ is a pointer to a node whose \var{timestamp}
%field is either TBD or stores a timestamp that is less than or equal to  
%S.timestamp at the time that the $O$'s constructor is invoked. 
\end{definition}

Let $\delta$ be any execution of \OptVCAS\ on $O$.
By inspection of the code, when $O$ is created, the constructor of $O$
calls initTS on the node $nd$ pointed to by the initial value of $O$. This implies that 
the timestamp of $nd$ has been set before any operation is performed on $O$. 
To define the version list of $O$, we find it useful to assign $O$ a {\em timestamp}. 
Specifically, the timestamp of $nd$ (i.e., the timestamp of the node that serves as the initial value of $O$) 
serves also as the timestamp of $O$.
%We assume that the \ovCAS\ object has a timestamp associated with it which is the timestamp
%of the Node it points to. We assume that 

We  prove that \OptVCAS\ is linearizable under the following assumption.
%if $O$ is a distinct-values \vCAS\ object.
%The proof requires to make the following assumption.

\begin{assumption}
\label{asm:opt}
	1) $O$ is a distinct-values \vCAS\ object,
2) whenever \ovrsnap($ts$)\ is executed on $O$, $ts$ has a value which is greater than or equal to the timestamp
of $O$,
and 3)  the initial value of $O$ is a pointer to a node whose \var{timestamp}
field is either TBD or stores a timestamp that is less than or equal to  
S.timestamp at the time that the $O$'s constructor is invoked.
\end{assumption}

We later prove that Assumption~\ref{asm:opt} 
is satisfied for every \vCAS\ object that is implemented using \OptVCAS\ 
in $OptD'_2$.

The version list of $O$ at a configuration $C$ of $\delta$ is the list of Nodes we get
if we start from the Node pointed to by $O.Head$ at $C$ and follow \var{nextv} pointers 
until we reach a Node whose timestamp is less than or equal to the timestamp 
of $O$.
%(we include the node we stop in the version list only if its timestamp is equal to $O$'s timestamp
%and it is not a dummy NULL node).
Since $O$'s timestamp is greater than or equal to the timestamp of the last Node in $O$'s version list, 
Assumption~\ref{asm:opt} implies that \ovrsnap\ always terminates by returning a Node in $O$'s version list
(i.e., it never follows the \var{nextv} field of the last node in $O$'s version list).
\Youla{Note that the last node may have timestamp which is smaller than $O$'s timestamp.
Take this in consideration when later prove correctness.}

By inspection of the pseudocodes of \VerCAS\ and \OptVCAS, we observe that there is a straightforward analogy
between the code executed on each line of \VerCAS\ and the code executed on the corresponding line of \OptVCAS\ (see lines 19-55 of the algorithms).
The only differences between the two algorithms is that the version list of $O$ created by executing \OptVCAS\
%created in \OptVCAS\ 
is a list of Nodes, whereas the version list of $O$ created by executing \VerCAS\ %created by \VerCAS\ 
is a list of VNodes
whose \var{val} fields store pointers to Nodes. Therefore, \var{Head} is a pointer to a Node,
whereas \var{VHead} is a pointer to a VNode, and the same is true for other local pointer variables
in the different routines that point to records (of type Node or VNode) of the version list of the object each time.

The similarity of the two algorithms, 
makes it easy to prove that \OptVCAS\ is linearizable (given that Assumption~\ref{asm:opt}), 
by following the same proof technique as for \VerCAS. Specifically, we first assign linearization points to operations
of \OptVCAS\ in a way similar we assign linearization points for \VerCAS\ and then 
prove a sequence of claims (Theorems, Lemmas, etc.) that are similar to the claims
necessary in Section~\ref{sec:vcas} for proving the correctness of \VerCAS.



\remove{
------------------------------------------
\Youla{What follows requires more work.}

\Youla{I have changed slightly the order in which the material appears in what follows to solve some problems in the correctness proof of the 
unoptimized version:
Also we have to prove that lin points are well-defined. This means that some lemmas
may need to be moved earlier.
We have to define what the "current value of a linearizable \vCAS\ (\ovCAS) implementation is in the Model section.}

By inspection of the pseudocode, it follows that the following claims hold. 

\begin{lemma}
\label{lem:initTS opt}
The following hold:
\begin{enumerate}
\item
Every successful \CAS\ on Line~\ref{line:casTS} makes valid the timestamp of a distinct Node.
\item
After a complete execution of \var{initTS} on some Node \var{n}, \var{n->ts}
stores a valid timestamp.
\item \func{initTS} can only be executed on Nodes that are in the version list of $O$.
\end{enumerate}
\end{lemma}

%\textbf{Linearization Points.} 
%We will show in Lemma \ref{lem:cur-val} that whenever \var{Head} points to a node whose timestamp is valid, $Head$ stores the current value of the \ovCAS{} object. 
Linearization points to operations are asigned as follows:

% Defining linearization points of \vcas based on return points are not ideal because incomplete vcas operations should be linearized as well.
\begin{itemize}
  \item An \ovcas(\var{oldV}, \var{newV}) operation $op$ is linearized depending on the line it returns.
	  If it returns on Line \ref{line:vcas-true2}, then it successfully appends a node $n$ to the version list and it is linearized on Line~\ref{line:readTS} of the \var{initTS} method that makes the timestamp of $n$ valid. 
  Let $h$ be the value of \var{Head} read at Line \ref{line:vcas-head} by the \ovcas{} operation.
  If $op$ returns on Line \ref{line:vcas-false1} or \ref{line:vcas-true1},  then it is linearized at the first configuration during the \ovcas{} operation where \var{Head} equals $h$ and the timestamp of $h$ is valid. 
		Since $op$ calls \initTS\ on Lines~\ref{}49 and~\ref{}44,
		Lemma~\ref{lem:initTS opt} implies that these linearization points are well-defined.
		Finally, if $op$ returns on Line \ref{line:vcas-false2}, then we later prove (Lemma~\ref{++}) that there is at least one other \ovcas{} operation that is linearized in the execution interval of $op$ and writes a value that is not equal to \var{oldV}.
		Then, $op$ is linearized immediately after the linearization point of the first such \ovcas{} operation (ties are broken arbitrarily).

  \item Consider any \ovrd{} operation $op$ and let $h$ be the value of \var{Head} read by $op$ on Line \ref{line:readHead}.
  Operation $op$ is linearized at the first configuration during the \ovrd{} operation where \var{Head} equals $h$ and the timestamp of $h$ is valid. 
  Since $op$ calls \initTS\ on Line~\ref{}39,
  Lemma~\ref{lem:initTS opt} implies that this linearization point is well-defined.

  \item Any \ovrsnap{} operation is linearized at its last step. \Hao{maybe linearized \readss{} similar to \vrd{} to reuse lemmas.}

  \item Consider any \ovtsnap{} operation $op$ and let $t$ be the value read by $op$ from \var{timestamp} on line \ref{line:read-time}.
 Operation $op$ is linearized when the value of \var{timestamp} changes from $t$ to $t+1$.
\end{itemize}

We argue that similar lemmas as those proved for \VerCAS\ hold for \OptVCAS. 
We summarize the statements of those lemmas below and explain the differences
in the proof (if any). 


\begin{lemma}
\label{lem:lin-head opt}
  When a modifying \ovcas{} operation $V$ is linearized, \var{Head} points to the Node pointed to by the $newV$ argument of $V$.
\end{lemma}

\begin{lemma}
\label{lem:cur-val opt}
At any configuration at which \var{Head->ts} is valid, \var{Head} stores the current value of the \ovCAS{}.
%if \var{VHead} points to a node $n$ whose timestamp is valid, then $n.val$ stores the current value of the \vCAS{} object.
\end{lemma}

\begin{lemma}
\label{lem:headInvalid opt}
In every configuration $C$, only the Node pointed to by \var{Head} in the version list of $O$ 
may have an invalid timestamp. All other Nodes in the version list have valid timestamps.
\end{lemma}


\begin{lemma}
\label{lem:head-valid opt}
If a process reads a pointer $h$ from \var{Head} and then calls \initTS{} on $h$, 
there exists a configuration between the read and the end of the \initTS{} such that \var{Head} points to $h$ and the timestamp of $h$ is valid.
\end{lemma}

\begin{observation}
\label{obs:lin-after-append opt}
Each modifying \ovcas{} operation is linearized after it performs Line \ref{line:append}.
\end{observation}

\begin{lemma}
\label{lem:linorder opt}
The linearization point of each operation lies within its execution interval.
\end{lemma}

\begin{observation}
\label{obs:ts-valid opt}
Consider a \var{Node} $n$ that was appended by a modifying \ovcas{} $V$.
If the timestamp of $n$ is valid, then $n$.\var{ts} stores the value of \var{S.timestamp} at the linearization point of $V$.
\end{observation}

\begin{lemma}
\label{lem:vsclp opt}
The modifying \ovcas\ operations are linearized in the order they append Nodes in the list.
\end{lemma}

These imply that the following theorem holds:
}



\begin{theorem}
	\label{th:optvcas}
\OptVCAS\ is a linearizable implementation of a \vCAS\ object of distinct values.
\end{theorem}


\myparagraph{{\bf Correctness of $OptD'_2$}}
Since $D'$ is a recorded-once concurrent data structure,
$OptD'_2$ is also a recorded-once implementation.
%Let $\alpha$ by any execution of $OptD'_2$. 

Consider any execution $\alpha$ of $OptD'_2$. 
We refer to $\alpha$ in what follows.
%Our first lemma proves that Assumption	\ref{asm:opt} holds


\begin{lemma}
\label{lem:asm}
Assumption~\ref{asm:opt} holds 
for all \vCAS\ objects that are implemented using \OptVCAS\ in $OptD'_2$. 
%
\end{lemma}

\Youla{I consider what is called Proofs below to be more proof sketches. Also, they require more work.}

\begin{proof}
An immediate consequence of the fact that $OptD'_2$ is a recorded-once implementation,
is that every \vcas\ object that is created in any of its executions
(and therefore also those that are implemented using \OptVCAS) is a distinct-values object.
Thus, item 1 of the assumption holds.

We continue to argue that item 2 also holds.
Consider any \vCAS\ object $O$ in $\alpha$.
Whenever \ovrsnap($ts$)\ is executed on $O$ in $\alpha$, 
$ts$ has a value which is greater than or equal to the timestamp of $O$.
When $O$ is initialized to $v$, $v$ is a Node that has been already created and therefore its timestamp
has been set. This implies that the timestamp of $O$ is at least as high as $S.timestamp$
at the time of $O$'s creation. Since $O$ is a recorded-once  We will show that all nodes in the data structure
that point to this Node, have timestamps that are greater than or equal to $O$'s timestamp.
This is so, because the initialization of a Node's \vCAS\ objects occurs before the 
Node is inserted in the list. So, the timestamps of the Node is set later than the timestamps of its \vCAS\ objects,
and therefore, the timestamp of the Node is greater than or equal to the timestamps of its \vCAS\ objects.
%The same is true for the timestamps of the entry points to the data structure which will be . 

Consider a query that has a timestamp less than $O$'s timestamp. 
We argue that this query can never reach $O$, so it never applies 
\ovrsnap\ on it. This is so because the timestamp of the Node in which a pointer
to $O$ is recorded is larger than or equal to the timestamp of $O$,
and therefore if the query arrives to this Node it will traverse its version list
until it find a Node with timestamp less than or equal to its own timestamp
and therefore it will not access $O$. 

Finally, we argue that item 3 holds. \Youla{Yet to be written...}
\end{proof}

\begin{lemma}
\label{lem:last-node}
Consider two \vCAS\ objects $O_1$ and $O_2$ in $\alpha$. If a Node other than the last
in the version list of $O_1$ is contained in the version list of $O_2$, then it is the last
Node of $O_2$'s version list.
\end{lemma}

\begin{proof}
Since all Nodes are recorded-once, every \ovcas\ operation on any \vCAS\ 
object stores a distinct value. This means that every time an \ovcas\
is executed (on any \vCAS\ object), it writes a pointer to a newly allocated Node. Thus, the only
way for a Node $nd$ other than the last in the version list of $O_1$, 
to appear in the version list of $O_2$,
is if a pointer to $nd$ were used as the initial value of $O_2$. Therefore $nd$ is the last
Node in $O_2$'s version list.
\end{proof}

\begin{lemma}
\label{lem:ovrsnap-traverse}
Consider any \vCAS\ object $O$ in $\alpha$. 
No invocation of \ovrsnap\ on $O$ traverses the
\var{nextv} pointer of the last Node in the
version list of $O$.
\end{lemma}
\Youla{See whether this can be a corollary of Lemma 24.}

\begin{proof}
\Youla{Yet to be written...}
\end{proof}

% \Hao{What happens if initial is a new Node? when does its timestamp get set?}

Lemmas~\ref{lem:last-node} and~\ref{lem:ovrsnap-traverse} imply that the version lists 
of \vCAS\ objects are operated as if they are disjoint. This and Theorem~\ref{thm:opt1} 
allows us to argue that $\alpha$ is also linearizable.

\Youla{It would be good if we could add pieces of the proof that are missing here.}

\begin{theorem}
$OptD'_2$ is a directly linearizable implementation of $A'$.
\end{theorem}

\myparagraph{{\bf Example}} \Youla{Add material about \NBBST\ here.}

\vspace*{.5cm}
-----------------------------------

Observations that might help for proof:

\begin{itemize}
  \item Nodes can be shared between multiple \vCAS{} operations
  \item Once \vnext{} and \ts{} is set, they can't be changed
  \item A \vcas{} might linearize due to an operation on a different \vCAS{} object.
  \item To construct the version list of a \vCAS{} object, we look at the set of nodes that it ever pointed to and arrange them in order. We probably want to show that the version pointers are consistent with this sequence.
  \item For each \vCAS{} object, its initial node's version pointer will never be accessed by operations on that object. This is important because the initial node's version pointer is actually part of another \vCAS{} object. It is meaningless for this \vCAS{} object.
  \item All the timestamps in a \vCAS{} object's version list are "correct" except for the initial node, who's timestamp is lower than what it should be. It's ok for the initial node's timestamp to be lower because a \vrd{} operation will never traverse past that node anyways.
  \item Need to prove that NULL initial values are properly handled.
\end{itemize}



\begin{figure*}
\begin{minipage}[t]{.43\textwidth}
  \begin{lstlisting}[linewidth=.99\columnwidth, numbers=left]
using @\hl{Value = Node*}@;  

class Snapshot {
  int timestamp;
  Snapshot() { timestamp = 0; }   @\label{line:ss-con-opt}@
  int takeSnapshot() {
     // same as in VerCAS}

Snapshot S;  // global snapshot object

class Node {
/* other fields of 
   Node struct of D */
  ...
  @\hl{Value nextv;}@
  @\hl{int ts;}@
};

class OptVersionedCAS {
  @\hl{Value Head;}@


  OptVersionedCAS(Value v) {
    @\hl{Head = v;}@
    initTS(Head);  }

  void initTS(@\hl{Value n}@) {
    if(n->ts == TBD) {
      int curTS = S.timestamp;
      CAS(&n->ts, TBD, curTS); } }
\end{lstlisting}
\end{minipage}\hspace{.3in}
\begin{minipage}[t]{.52\textwidth}
\StartLineAt{31}
\begin{lstlisting}[linewidth=.99\textwidth, xleftmargin=5.0ex, numbers=left]
  Value OptreadSnapshot(int ts) {
    @\hl{Value node = Head;}@
    initTS(node);
    while(node->ts > ts) node = node->nextv; 
    return @\hl{node}@; }

  Value OptvRead() {
    @\hl{Value head = Head;}@
    initTS(head);
    return @\hl{head}@; }

  bool OptvCAS(Value oldV, Value newV) {
    @\hl{Value head = Head;}@
    initTS(head);
    if (head != oldV) return false;
    if (newV != oldV) return true;
    @\hl{newV->nextv = oldV; newV->ts = TBD;}@
    if(CAS(&Head, head, newV)) {
      initTS(newV);
      return true; }
    else {
      // Val can't be NULL
      initTS(Head);
      return false; } }
};
  \end{lstlisting}
\end{minipage}
\caption{Linearizable implementation of a \vCAS{} object without indirection where \vrd$(\infty)$ and \vcas{} take constant time. Major differences between this and Figure \ref{fig:vcas-alg} are highlighted.
%\Yihan{in vCAS why don't we compare oldV and head?}
%\Hao{Good point, should be fixed now}
}
\label{fig:vcas-direct-alg}
\end{figure*}



%\Hao{Should the pseudo-code be Object.function() or function(Object: pointer to)? I should look at exampels from PODC to see what their style is. Also, in the definition of VerLLSC, we should make the definition of the global timestamp more concrete.}

%\Hao{Given the restriction that newV has to be a new node, that makes implementing SC trivial. In the other case, the level of indirection made implementing SC trivial.}

%\Hao{Need to define what "new Node" means. It can be used by a previous unsuccessful SC, but it can't have been used by a successful SC. Not sure if this is an accurate definition.}



==> prelim.tex <==
% !TEX root = main.tex

\subsection*{Preliminaries}
\label{sec:prelim}
% Guy : moved most of this section to the file appendixprelim.tex

We use the standard
definition of \emph{linearizable}~\cite{herlihy1990linearizability}, which roughly states that
every operation must appear to have taken effect atomically between
its invocation and response.   This is formalized along with our proofs in
the Appendix.
A subset of the operations are wait-free in an implementation if they have this property.
The {\em step complexity} of an operation instance $op$ invoked by a process $q$ in an execution
is the number of steps $q$ performs from $op$'s invocation to is response.
The {\em step complexity} of an operation is the maximum step complexity of any instance
of the operation in any execution.



==> removal.tex <==
\subsection{Splicing Nodes Out}
\Note{The optimized version will likely sound much more like Eric and Youla's persistent tree from SPAA. For that, we believe that splicing out nodes from version lists is the same as in the general construction (reduces to splicing nodes out from a linked list), but that requires some proof, since it doesn't look like linked-lists. Below are our (partial) notes on how to splice out nodes from Eric and Youla's tree. In particular, this part argues why we only need to care about 2 `parents' for each node, but we believe we can reduce that further to just 1 `parent', thereby arriving at a doubly linked list.}


Once a node is identified by the RSQ as ready to be removed, we have to actually physically remove it from the data structure.
If each node only had one parent, splicing a node $n$ out would be easy; we would simply swing $n$'s parent's child pointer from $n$ to $n$'s child. \Yihan{Not sure if we should call it $n$'s child. It is actually the next version of $n$ (or the ``replacement'' as defined below.} We would just need to know who $n$'s parent is. It is easy to maintain a backpointer from $n$ to $n$'s parent for this purpose.

However, nodes may have multiple parents in the persistent tree, since maintaining the previous versions of each node means that the structure becomes a DAG. In fact, every time a node's `uncle' in the tree is deleted, that node gains another parent. Thus, a node could have as many parents as its original depth in the tree.
This can cause problems when trying to splice out a node; do we need to change the child pointers of all of its parents? If so, how do we find these parents?

We first introduce some terminology.

To be able to reason about this DAG, we consider its state at a time $t$, and separate it into two parts; the \emph{current tree}, and the \emph{history}. The current tree at time $t$ refers to nodes that can be traversed by a reader that starts at time $t$. That is, these are the nodes of the tree that are reachable without traversing any \emph{prev} pointer. The \emph{history} consists of all nodes that are not in the \emph{current tree}.

We partition the edges in the tree into two types: \emph{child} pointers, and \emph{prev} pointers. Child pointers are pointers from the tree data structure, and prev pointers are those used inside \emph{version lists}. If node $p$ points to node $n$ through a child pointer, we say $p$ is $n$'s \emph{parent}. If $p$ points to $n$ through a prev pointer, we say $p$ is $n$'s \emph{replacement}. Note that the replacement of $n$ is the only node that points to $n$ with a \emph{prev} pointer.

\begin{observation}\label{obs:history}
	No node $n$ in the history part of the DAG can be accessed by traversing from any node $c$ in the current tree without passing through at least one prev pointer.
\end{observation}

We call the first parent that a node $n$ has in the tree $n$'s \emph{original parent}. Note that $n$'s original parent might now always be a parent of $n$ because the orignal parent can change to point to another child.


%We first note that each node only ever transitions from being in the \emph{current tree} to being in the \emph{history} once. Once a node is in the \emph{history} part of the DAG, it never goes back to being in the current tree.
%Furthermore, a node $n$ gains exactly one new parent upon its transition into the history set; we call this parent its \emph{replacement}.
%Note that the replacement of $n$ is the only node that points to $n$ with a \emph{prev} pointer. Note also that once a node enters the history set, it never gains any other parents.

We now present a sequential algorithm for splicing out a node $n$ that has been returned by an RSQ. We later discuss how to make this algorithm safe in a concurrent setting. Note that if $n$ is returned by an RSQ, then $n$ must be in the history of the DAG. This is because $n$'s lifetime must be over for an RSQ to return it.

\begin{lstlisting}[caption = Disconnection Algorithm, label=alg:splice]
	When a node @$n$@ is inserted into the data structure, include a field in @$n$@ 
    pointing to @$n$@'s parent.
	This field is called the @\emph{original parent back pointer}@.
	When a node @$n$@ is replaced, include a field in @$n$@ pointing to @$n$@'s replacement.
	This field is called the @\emph{replacement back pointer}@.
	When node @$n$@ is returned by an RSQ:
		for each back pointer @$b$@ of @$n$@:
			follow @$b$@ to node @$p$@.
			If @$p$@ has a child pointer or prev pointer @$ptr$@ pointing to @$n$@,
				swing @$p.ptr$@ from @$n$@ to @$n.ptr$@.
		zero out all original parent back pointers that point to @$n$@
\end{lstlisting}

Notice that we only ever set at most 2 back-pointers for any node $n$: a back pointer to its original parent, and a back pointer to its replacement. Therefore, for Algorithm~\ref{alg:splice} to be correct, we must show that if $n$ is returned by an RSQ, $n$ can never be reached by traversing a pointer to it from any node other than these two.

To do so, we denote by $n.ts$ the timestamp of node $n$, and by $n.endts$ the end of $n$'s lifetime. We show the following invariants, which hold regardless of how many times we execute Algorithm~\ref{alg:splice}.

\begin{enumerate}
	\item \label{inv:OPts} If $n$'s original parent is $p$, then $n.ts \geq p.ts$.
	\item \label{inv:ptrts} If at any point in time, $p.child = n$ and $n.ts > p.ts$ then $n$'s original parent is $p$.
	\item \label{inv:noaccess} If an RSQ returns node $n$ at time $t$, then at any time $t' \geq t$, $n$ can't be accessed other than through its original parent or a prev pointer.
	\item \label{inv:sharedOP} Let $p$ be the original parent of $n$. Then for all $m$ in $n$'s version list (all nodes $m$ that are reachable from $n$ by traversing only prev pointers), if $m.ts > p.ts$, then $p$ is $m$'s original parent.
\end{enumerate}

\begin{proof}
	Note that in the algorithm of the persistent tree from SPAA, all pointer swings are always to new nodes, and new nodes always have a timestamp that is greater than or equal to all existing nodes.
	
	Invariant~\ref{inv:OPts} is easy to see, since if $p$ is the original parent of $n$, then $n$ was a new node when $p$ became its parent, and therefore has a timestamp that is greater than or equal to $p$'s timestamp. This holds regardless of executions of Algorithm~\ref{alg:splice}, since Algorithm~\ref{alg:splice} does not affect original parent relationships.
	
	We prove the rest of the invariants by induction on the number of times Algorithm~\ref{alg:splice} is run.
	
	\textsc{Base case.} If Algorithm~\ref{alg:splice} has never been run, we show that these invariants hold in the original persistent data structure.
	
	Invariant~\ref{inv:ptrts}: We want to show that if $p$ is not $n$'s original parent, but at some point in time $p$ was $n$'s parent, then $p$ was inserted into the data structure after $n$. Assume by constradiction that $p$ was inserted into the data structure before $n$. Then $p$ must have become $n$'s parent by a pointer swing of one of $p$'s child pointers to $n$. However, pointer swings only swing to new nodes. So in this case, $p$ must be $n$'s original parent. This contradicts the assumption that $p$ is not $n$'s original parent.

	Invariant~\ref{inv:noaccess}: Let $p$ be a non-original parent of $n$, and let $n$ be returned by RSQ at time $t$. Then by Invariant~\ref{inv:ptrts}, we know that $p.ts \geq n.ts$. Furthermore, we know that at time $t$, $n$ must be part of the history. Let $t'$ be the time at which $n$ became part of the history. In the original persistent data structure, once $n$ becomes part of the history, it cannot gain any
	new parents, so $p$ must have existed and had a child pointer that points to $n$ at time $t'$. By Observation~\ref{obs:history}, $p$ must also be a part of the history at time $t'$. Therefore, $p.endts \leq n.endts$. Thus, $p$'s lifetime is contained within $n$'s lifetime. Therefore, if an RSQ returned $n$, then $p$ must also be safe to return in an RSQ. In particular, this means that no thread will ever stop at $p$, and therefore no thread will ever reach $p$'s children through $p$'s child pointer.
	
	Invariant~\ref{inv:sharedOP}: Assume that $p$ is $n$'s original parent, $n$ is $m$'s replacement, and $p.ts \leq m.ts$.  Note that since $n$ is $m$'s replacement, $m$ must have been $p$'s child at the time when $n$ was inserted. Since $m$ was $p$'s child, and by Invariant~\ref{inv:ptrts}, $p$ must have been $m$'s original parent as well.

	\textsc{Inductive step.} Invariant~\ref{inv:OPts} is not affected by executions of Algorithm~\ref{alg:splice}, so it holds no matter
	how many times the algorithm is run. Simiarly, each version list can only shrink due to Algorithm~\ref{alg:splice}, so
	Invariant~\ref{inv:sharedOP} also holds no matter how many times the algorithm is run.

	% Suppose Invariant \ref{inv:ptrts} hold after $k-1$ executions of Algorithm~\ref{alg:splice}, we will show that it holds after $k$ executions of Algorithm~\ref{alg:splice}.

	For Invariant \ref{inv:ptrts}, suppose the $k$th execution of Algorithm~\ref{alg:splice} changes $p$'s child pointer from
	$n$ to $n.prev$. This can only happen if $p$ is $n$'s original parent. There are two cases, either $n.prev.ts \leq p.ts$
	in which case Invariant \ref{inv:ptrts} does not apply to this newly added child pointer, or $n.prev.ts > p.ts$ in which case
	by Invariant \ref{inv:sharedOP}, $p$ is $n.prev$'s original parent and Invariant \ref{inv:ptrts} holds on this new child pointer.

	Finally, we turn our attention to Invariant \ref{inv:noaccess}. Let $p$ be a non-original parent of $n$, and let $n$ be returned by RSQ at time $t$. Then by Invariant~\ref{inv:ptrts}, we know that $p.ts \geq n.ts$. Furthermore, we know that at time $t$, $n$ must be part of the history. Let $t'$ be the time at which $n$ became part of the history and let $t_p$ be the time at which $p$ became a parent of $n$. If $t_p < t'$, then after time $t$, by the same argument as the base case, no thread will follow this pointer from $p$ to $n$.
	Suppose $t_p > t'$. Let $m$ be $n$'s replacement at $t_p$. Then the pointer from $p$ to $n$ must have been set by an execution of Algorithm \ref{alg:splice} that removed $m$. Since $p$ is not $n$'s original parent, this pointer swing can only happen if all of
	the nodes who's original parent is $p$ have been removed. However, $p$'s lifetime is contained in the lifetime of these nodes
	which means that $p$ is safe to return from the RSQ datastructure at time $t_p$. Therefore, none of $p$'s child pointers can be followed
	after time $t_p < t$, which completes the proof of invariant \ref{inv:noaccess}.
\end{proof}

Invariant \ref{inv:noaccess} implies that Algorithm~\ref{alg:splice} is correct because the invariant says that the node $n$ being
removed can only be access through its original parent or its replacement and the algorithm forwards both those pointers. 

==> snapshot.tex <==
% !TEX root =  main.tex

\section{Snapshots and Queries}
\label{sec:snap-query}

\Eric{A lot of what I've written here will eventually be moved to the appendix, I expect.}

Using our \vCAS{} objects from Section \ref{sec:vcas}, we can add snapshot and query operations to a wide range of concurrent data structures.
Recall from Section \ref{sec:prelim} that snapshots provide a consistent view of the low-level  state of the concurrent data structure at some configuration, whereas queries are read-only operations on the abstract data type implemented by the data structure. Range query and predecessor queries are examples of query operations on a set ADT.

After some preliminaries in Section \ref{sec:linearizable}, we show in \ref{sec:query}
how to add support for queries to concurrent data structures built using \CAS\ objects
by taking a snapshot of the data structure.


\subsection{Modelling Linearizability}
\label{sec:linearizable}

\Eric{This may belong in a model section instead of here}

Let $P$ be a set of processes.
Our construction assumes that we have a linearizable concurrent data structure $D$ that
implements an abstract data type $A$.  $A$ can be defined by a sequential
specification $(Q_A,\Ops,\Res,\delta)$, where
\begin{itemize}
\item
$Q_A$ is a set of states,
\item
$\Ops$ is a set of operations that can be performed,
\item
$\Res$ is a set of responses that can be returned as the response to an operation, and
\item
$\delta$ is a transition function that maps pairs in $Q_A\times Ops$ to non-empty subsets of $Q_A\times \Res$.
\end{itemize}
The transition function, like all functions mentioned in this paper, is assumed to be computable.
This sequential specification describes how $A$ behaves when it is accessed by one operation at a time.
In particular, if $(q',\res)\in \delta(q,op)$, it means that if operation $op$ is performed on $A$
when $A$ is in state $q$, a legal outcome is for $op$ to return the response $\res$ and
move $A$ into state $q'$.  This definition allows $A$ to behave non-deterministically.
A {\it sequential history} of $A$ for the set of processes $P$ is a sequence of the form
$q_0, (p_1, op_1, \res_1), q_1, (p_2, op_2, \res_2), q_3, \ldots$ where for all $i$, $(q_i,\res_i)\in \delta(q_{i-1},op_i)$ and $p_i\in P$.


We can model an implementation $D$ of $A$ for a set of processes $P$ as an I/O automaton $(Q_D, \Int, \Ext, \Steps, \Init)$ where
\begin{itemize}
\item
$Q_D$ is a set of configurations,
\item
$Int$ is a set of internal actions,
\item
$Ext$ is a set of external actions in which a process either invokes or completes an operation of $A$, namely $Ext = \{invoke(p,op) : p\in P, op\in \Ops\} \cup \{return(p,\res) : p\in P, \res\in \Res\}$,
\item
$Steps\subseteq Q_D \times (\Int \cup \Ext) \times Q_D$, and
\item
$\Init:Q_A \rightarrow Q_D$ describes, for each possible state of $A$, how to initialize~$D$.
\Eric{Or should we just assume, for simplicity, a fixed initial state for $A$ and for the implementation $D$?}
\end{itemize}
In a shared-memory system, a configuration is intended to represent the state of shared memory and all processes' local states (including each process's programme counter).
If $(C,act,C')\in \Steps$, it means that when the implementation is in configuration $C$, the action $act$ is enabled and would take the system from $C$ to configuration $C'$.
We assume each internal action corresponds to the execution of an instruction in the code of a single process that includes at most one access to shared memory.  Such an action cannot
modify the local state of any other process.
Moreover, we assume that each process $p$'s local state is {\it idle} in $\Init(q_0)$ for any $q_0\in Q_A$.  The only actions by $p$ enabled when $p$'s state is {\it idle} is are
$invoke(p,*)$ actions. A $return(p,*)$ action makes $p$'s state idle and no other actions can change $p$'s state to idle.

An execution of $D$ is an alternating sequence of configurations and actions $C_0, act_1, C_1, act_2, \ldots$ such that $(C_{i-1}, act_i, C_i)\in Steps$ for all $i$.
By the assumptions related to the behaviour of a process $p$'s idle state, the subsequence consisting of external actions of $p$ alternate between $invoke$ and $return$ actions, starting with an $invoke$.  We say that the next $return(p,*)$ action after an $invoke(p,*)$ {\it matches} that $invoke$ action.  Internal actions by $p$ can only occur between an $invoke(p,*)$ and its matching $return(p,*)$.

One way to show that $D$ is a linearizable implementation of $A$ is to define linearization points for all operations.  More formally,
if $\alpha$ is an execution, an {\it annotation $\alpha'$ of $\alpha$} is
a sequence obtained from $\alpha$ by inserting linearization points of the form
$lin(p,op,res)$, where $p\in P$, $op\in Ops$ and $res\in Res$.

\begin{definition}
\label{def:linearization}
We say that an annotation $\alpha'$ of $\alpha$ is a {\it linearization} of $\alpha$ starting from initial state $q_0$ if there exists a sequential history $q_0, (p_1, op_1, \res_1), q_1, (p_2, op_2, \res_2), q_3, \ldots$ of $A$ such that,
\begin{itemize}
\item
between each $invoke(p,op)$ and its matching $return(p,res)$ action in $\alpha'$, there is exactly one $lin(p,op,res)$,
\item
for any $invoke(p,op)$ in $\alpha'$ that has no matching $return$ action, there is
at most one $lin(p,op,*)$ after that $invoke$ action,
\item
there are no other linearization points in $\alpha'$,
\item
for all $i$,
the $i$th linearization point in $\alpha'$ is $lin(p_i,op_i,res_i)$, and
\end{itemize}
\end{definition}

We say the implementation $D$ of $A$ is {\it linearizable} if, for all $q_0\in Q_A$,
every execution $\alpha$ of $D$ that starts from the configuration $\Init(q_0)$
has an annotation $\alpha'$ that is a linearization of $\alpha$ starting from $q_0$.
\Eric{I claim this is equivalent to the standard definition of linearizability.}

\Eric{Add some glue to informally introduce and motivate direct linearizability; check Herlihy Wing paper that defined linearizability to see how our definition of direct linearizability compares to what they talk about in Section 4}

For a configuration $C$ of $D$, let $\hat{C}$ denote the state of the shared memory in $C$.
(Recall that $C$ consists of the state of shared memory, together with the internal states of all processes.)  Let $\hat{Q}_D = \{\hat{C} : C\in Q_D\}$.
An abstraction function allows us to look at the state of the shared memory of the
concurrent implementation $D$
and figure out what state of the ADT $A$ it represents.  This interpretation of the
shared memory's state
must be consistent with some linearization of every history.  We formalize this
notion in the following definition.

\Yihan{Although using $C$ for a configuration looks standard, in other parts of the paper we are using lowercase letters for elements in a set and uppercase letters for sets, e.g., a state $q$ in set of states $Q$. This does not seem to be a huge problem but sometimes can be confusing. Should we consider using another notation, maybe something like $d_C$?}

\begin{definition}
\label{def:abs}
An \emph{abstraction function} from $D$ to $A$ is a function $F: \hat{Q}_D\rightarrow Q_A$ that satisfies the following properties for all $q_0\in Q_A$:
\begin{itemize}
\item
$F(\widehat{\Init(q_0)})=q_0$, and
\item
for all executions $\alpha$ of $D$ that start from configuration $C_0=\Init(q_0)$, $\alpha$ has a linearization $\alpha'$ corresponding to some
sequential history $q_0, (p_1, op_1, \res_1), q_1, (p_2, op_2, \res_2), q_3, \ldots$ of $A$
such that, for any prefix of $\alpha'$ that contains $m$ linearization points and ends in
a configuration $C$, $f(\hat{C}) = q_m$.
\end{itemize}
\end{definition}

We examine some consequences of the definition.
If, in some linearization $\alpha'$, there are no linearization points placed between two configurations $C_i$ and $C_j$, then $F(\hat{C_i}) = F(\hat{C_j})$.
If, between two consecutive configurations
$C_i$ and $C_{i+1}$ in some linearization $\alpha'$, there is a sequence $\gamma$ of linearization points, then
it must be possible to get from state $F(\hat{C_i})$ to state $F(\hat{C}_{i+1})$ in $A$
by performing the sequence of operations in $\gamma$, and the operations
should produce the same results as those specified in $\gamma$.

We claim that, quite often, linearization arguments for concurrent implementations
are done by building an abstraction function, or could easily be rephrased
to do so.
For example, consider the lock-free binary search tree of Ellen et al.~\cite{EFRB10}.
It implements a set ADT that supports insert, delete and find operations.
The elements of the set are stored in the leaves of a binary search tree.
For each insert and delete operation that successfully updates the set,
there is a single successful \cas\ instruction that updates one child pointer of a node
in the tree to add or remove a leaf containing the key being inserted or deleted.
That \cas\ instruction is used as the linearization point of the operation.
It is proved in \cite{EFRB10} that the data structure maintains as an
invariant that the items in the set ADT
correspond exactly to the items stored in the leaves of the tree.
This yields a natural abstraction function:
for any configuration $C$, $F(\hat{C})$ is the set of items
stored in leaves that are reachable from the root of the tree in $C$.
Each \find($k$) operation that returns true and each unsuccessful \insertop($k$) operation are
assigned linearization points when a leaf containing $k$ is known to be in the tree.
Similarly, \find($k$) operations that return false and unsuccessful \deleteop($k$) operations
are linearized when no leaf in the tree contains $k$.

The requirement that the abstraction function should only depend on the state
of the shared memory is also quite natural:  if the state of the ADT $A$ were to depend
on the states of the private memories of some of the processes, then it would not
be possible for a process to recover the state of the ADT if, for example, the processes
holding this key information died.

By definition, if there is an abstraction function from $D$ to $A$, then $D$ is a linearizable implementation of $A$. This justifies the following definition.

\begin{definition}
\label{def:direct}
$D$ is a {\it directly linearizable} implementation of $A$ if there is an abstraction function from $D$ to~$A$.
\end{definition}


\Eric{Add some discussion of the relationship between strong linearizability and direct linearizability.  Can look into future when coming up with linearization, so more general
than strong linearizability.  I thought about whether the defn of direct linearizability
is equivalent to the existence of a refinement mapping from $D$ to the canonical automaton
associated with $A$, but I don't think it is, because with our defn, one can look into
the future when setting linearization points.}

\subsection{Adding Queries}

In this section, we show how to obtain a \emph{snapshot} of the shared memory of
a concurrent data structure based on \CAS\ objects and use it to add support for query
operations.
This requires transforming the original data structure to use our \vCAS{} objects in place of the regular \CAS{} objects.
This transformation preserves all existing
correctness guarantees (e.g., linearizability, strong linearizability,
sequential consistency) of the concurrent data structure, as well as all existing progress guarantees (e.g.,
wait-freedom, lock-freedom). The transformation also preserves any runtime
bounds that were proven for the original algorithm up to constant factors.
These properties hold regardless of how many snapshot operations are running
concurrently with original data structure operations. Furthermore, the new
query operations are wait-free.
The time complexity of a snapshot operation is bounded by the number of objects viewed by the snapshot, plus the number of \CAS\ operations concurrent with the snapshot.

A {\it query operation} on an ADT is one that never changes the state
of the ADT.  More formally, a query operation $op$ has the property that
for all states $q$ and for all $(q',res)\in \delta(q,op)$, $q'=q$.
Without loss of generality, we shall consider implementing deterministic
queries.  (If we can implement an arbitrary deterministic query,
we can also implement non-deterministic ones simply by choosing one
of the possible query results for each state.)
A deterministic query $op$ on an ADT $A$ defines a function
$R:Q_A\rightarrow Res$, where $R(q)$ is the unique response such that
$(q,R(q))\in \delta(q,op)$.

Suppose we add a set of query operations to the ADT $A$ to define a new augmented ADT $A'$.
Let $R_1, \ldots, R_k$ be the functions defined by the new query operations.
Given a directly linearizable implementation $D$ of $A$ that uses \CAS\ objects,
we describe how to construct a directly linearizable implementation $D'$ of $A'$
using \vCAS\ objects.
The new query operations will be wait-free, but not very efficient.
Later, we describe how to make the queries more efficient.

\Eric{Will have to update instructions to match new interface of versioned CAS object}
To obtain $D'$ we replace every \CAS\ object with a \vCAS\ object.
The implementation $D'$ also uses a single \snapshot\ object.
All \vCAS\ objects are  paired with this \snapshot.
Each \cas\ or \rd\ instruction on a \CAS\ object is replaced by a \vcas\ or \vrd($\infty$) on the corresponding \vCAS\ object.
All \vCAS\ objects in $D'$ are initialized in the same way as the
corresponding \CAS\ object in $D$
and the \snapshot\ object is initialized to have value 0.

To perform a new query operation of $A'$ whose result function is $R_i$, a process first reads the value of the \snapshot\ into a local variable \var{ts}. Next, it performs a \compinc(\var{ts}) on the \snapshot.
Then, it performs \rd(\var{ts}) instructions on all of the \vCAS\ objects to get a
global snapshot $S$ of the shared memory.
It then returns $R_i(F(S))$, where $F$ is the abstraction function from $D$ to $A$.

\begin{theorem}
$D'$ is a directly linearizable implementation of $A'$.
\end{theorem}
\begin{proof}
\Eric{This is a little informal because doing it even more formally would be deadly boring.}
Given a state $\hat{C}'$ of the shared memory of $D'$,
we can obtain a corresponding state $\hat{C}$ of the shared memory of $D$
by simply removing the \snapshot\ object; each \CAS\ object in $\hat{C}$ has the
same state as the corresponding \vCAS\ object in $D'$.
So we can define an abstraction function $F'$ from $D'$ to $A'$ in a natural way
by saying $F'(\hat{C}') = F(\hat{C})$.
We show that $F'$ is an abstraction function from $D'$ to $A'$.

Let $q_0$ be any state of $Q_A$ and let
$\alpha$ be an execution of $D'$ that starts from the initial configuration $C_0$ for $q_0$.
For convenience, we shall assume that $D$ includes a $null$ internal action such that
$(C, null, C)$ is a step for all configurations $C\in Q_D$; clearly, adding such a
null action to $D$ does not affect its linearizability.
Now, we can define an execution of $\beta$ that matches $\alpha$ step-by-step:
each action in $\alpha$ by a process performing a query operation  is changed to a
null action, and every other action is changed to the corresponding action of $D$
(with each \vcas\ or \rd($\infty$) changed to a regular \cas\ or \rd, respectively).
By the specification of \vCAS\ objects, $\beta$ is a valid execution of $D$.

By our assumption that $F$ is an abstraction function from $D$ to $A$, there is
an linearization $\beta'$ of $\beta$ and sequential history $q_0, (p_1, op_1, \res_1), q_1, (p_2, op_2, \res_2), q_3, \ldots$ of $A$ that satisfies Definition \ref{def:abs}.

We build a linearization $\alpha'$ of $\alpha$ by inserting into $\beta'$ linearization
points for each terminating query operation in $\beta$.
If a terminating
query operation $op$ reads the value $ts$ from the \snapshot\ object, then we insert $op$'s
linearization point immediately before the first \compinc($ts$) instruction.
(Such a \compinc\ exists, because the query itself performs one.)
Let $C'_{op}$ be the configuration of $D'$ immediately preceding this \compinc\ in $\alpha$.
Note that several query operations may be linearized together, prior to this \compinc,
since several query operations may read the value $ts$ from the counter.

According to the specification of \vCAS\ objects, all \vrd s performed by the query
will return the value of the \vCAS\ object in $C'_{op}$.  Thus, $op$ obtains $\hat{C}'_op$
by reading all memory locations. and then returns $F'(\hat{C}')$


\Eric{To be continued...}
\end{proof}

\begin{lemma}
Each new query operation of $A'$ is wait-free in $D'$.
\end{lemma}
\begin{proof}
\Eric{To be filled in.}

\Eric{I guess we need to say either the size of shared memory is finite, or
that we have some way of determining which \CAS\ objects have been written so far (e.g., a max register that records the index of the biggest CAS
object written so far).
Or, for pointer-based data structures, maybe we need a notion of reachable shared memory
and require that the abstraction function only depends on reachable shared memory.
}
\end{proof}

\begin{lemma}
If an operation of $D$ is obstruction-free, lock-free or wait-free, then the corresponding operation of $D'$ is too.
\end{lemma}
\begin{proof}
This claim follows immediately from Theorem \ref{thm:vcas}.
\end{proof}

\subsection{Making Queries More Efficient}

Quite often, the result of a query will not depend on the entire state of $A$, but
only on some part of it.  If it is possible to compute that part of the state
by only looking at a part of the state of $D$'s shared memory then a partial snapshot,
rather than a complete snapshot,
may suffice to answer the query.

\Eric{Add the stuff about the intermediate level.}

Look at some commonly used data structures and show how to design $A_Q$ operations for them. 

==> snapshot2.tex <==

\section{Supporting arbitrary queries}

% In Section \ref{}, we show how to modify common concurrent data structures so that they can support arbitrary queries. The techniques we present are fairly general and can be applied to other data structures as well.

\subsection{Snapshot Transformation}

\Hao{maybe get rid of snapshot transformation}

Given any concurrent data structure $D$ that is written using \rd{} and \cas{}, we show how to transform it into a new data structure $D'$ that supports snapshotting alongside all the operations originally supported by $D$. We call this our \emph{snapshot transformation}.

\begin{definition}
	\item 
\end{definition}

One important application of snapshotting is for adding queries to concurrent data structures, which we talk about more in the next section.
People have also found that snapshotting is valuble when debugging concurrent data structures \cite{trevor brown snapshot}.

\subsection{Queries}

We say that an operation is \emph{read-only} if it does not perform any CAS operations. \Hao{this probably belongs in prelims. We should mention that the algorithms we consider only access shared memory through read and CAS.}

Intuitively, a quiescently-linearizable operation is one that is correct when it is run on a snapshot of the concurrent state.

We say that a data structure $D$ supports a set of linearizable operations $L$ and a set of \emph{quiescently linearizable} operations $QL$ if $D$ is linearizable in all histories in which operations from $QL$ are run in isolation. These histories can contain invocation and responses for any operation in $L$ or $QL$, however once an operation from $QL$ is invoke, the process that invoked it is scheduled continuously until it returns a response. Note that operations from $QL$ can still happen during an operation from $L$, so they can still see an intermediate state of $D$.

In this paper, all the quiescently-linearizable operations are also required to be read-only. In Section \ref{}, we show that that any set of read-only, quiescently-linearizable operations can be made fully linearizable using our \vCAS{} objects.

It is not clear when it is possible to support read-only quiscently-linearizable operations or how hard it is to design these kinds of operations.
On one hand, they seem easier to design than linearizable operations because they don't need to worry about concurrent modifications.
On the other hand, they are read-only so they can't do helping.
In Section \ref{}, we show that many common concurrent data structures support a large set of quiescently-linearizable operations.

\subsubsection{Quiescent Query Transformation}

Given a concurrent data structure $D$ with a set of linearizable operations $L$ and a set of read-only, quiescently-linearizable operations $QL$, we can construct a linearizable data structure $D_\ell$ that supports operations from both $L$ and $QL$. 

The first step is to add a \timestamp{} object to $D$ and replace all \CAS{} objects with \vCAS{} objects. For each operation in $L$, we will replace each call to \cas{} with a call to \vCAS{} and each call to \rd{} with a call to $\vrd(\infty)$. 
Operations in $QL$ do not call \cas{}, so we just have to handle calls to \rd{}.
We insert a call to \snapshot{} at the beginning of each operation in $QL$ and store the timestamp it returns in a variable \var{ts}.
Then we replace each \rd{} operation with \vrd(\var{ts}).
This completes the transformation and we will call the resulting data structure $D_\ell$.

Given a history $H_L$ of operations from $D_\ell$. 


The resulting data structure we will call $D_\ell$ and it supports operations from both $L$ and $QL$.

Operations from $L$ have the same progress properties in $D_s$ as in $D$, and their runtimes are increased by only a constant factor. 

\Hao{specify linearization points and everything}

\begin{theorem}
	Given a concurrent data structure $D$ with a set of linearizable operations $L$ and a set of read-only, quiescently-linearizable operations $QL$, we can construct a linearizable data structure $D_s$ that supports operations from both $L$ and $QL$. Operations from $L$ have the same progress properties in $D_s$ as in $D$, and their runtimes are increased by only a constant factor. 

	Let $Q$ be an operation from $QL$ and let $C$ denote a configuration (aka concurrent state) of $D$.
	To give time bounds for $Q$, we assume that $Q$ accesses each CAS object a constant number of times. \Hao{Otherwise we would have to do caching. I don't know what the complexity of this would be in general.} 
	Let $s_Q(C)$ denote the runtime of $Q$ on configuration $C$ when $Q$ is run in isolation.
	In $D_s$, we will define the linearization point of $Q$ so that the runtime of $Q$ is $D_s$ is $O(s_Q(C_\ell) + W)$, where $C_\ell$ is the configuration at the linearization point of $Q$ and $W$ is the number of CAS operations concurrent with $Q$ that are on memory locations accessed by $Q$.
\end{theorem}

\subsubsection{\NBBST{} example}

In this section, we show how to add an arbitrary query $Q$ to the \NBBST{} as long as there is a sequential algorithm computing $Q$ on a regular, external BST.

A node in a regular BST consists of 4 fields: $key$, $val$, $left$, and $right$.
Note that if we take a state from the \NBBST{} and ignore all the marking and flagging fields, what we are left with is a regular, external BST.
We call this mapping from \NBBST{} state to external BST state $f_I$.
In the original \NBBST{} paper, \ins{} operations are linearized when the node it inserts becomes reachable and \del{} operations are linearized when the node it's trying to delete becomes unreachable from the root.
We keep the same linearization points.
Let $H$ be a low-level history resulting from a \NBBST{} execution and let $C$ be the state immediately after $H$.
Due to the way the linearization points are picked, the leaves in the external BST $f_I(C)$ represent exactly the nodes for which an \ins{} operation has linearized in $H$ but not a \del{}.
Therefore, if we pause a \NBBST{} execution at some configuration $C$ and run the sequential algorithm for $Q$ on the external BST state $f_I(C)$, this query will be linearizable with respect to \ins{} and \del{} operations.
Since $f_I(C)$ only ``hides'' information from $C$, we can run the sequential query on $C$ without computing $f_I(C)$ (e.g. the left child of a node in $f_I(C)$ is equal to the left child of a node in $C$).

We apply our snapshotting technique to make sure the sequential query sees a consistent state of the \NBBST{} even if it is being modified concurrently.
The first step is to replace all the \CAS{} objects in the \NBBST{} with \vCAS{} objects and add a global \timestamp{} object.
Next, for each call to \CAS{} in the \NBBST{}, we replace it with \vCAS{}, and for each call to \rd{}, we replace it with $\vrd(\infty)$.
Notice that this does not affect correctness because \vCAS{} and $\vrd(\infty)$ behave just like \CAS{} and \rd{}.
To implement $Q$ so that it is linearizable with respect to all the other operations, we begin by taking a \snapshot{} and storing the resulting timestamp in a variable \var{ts}.
Then we run the sequential algorithm for $Q$ except each time it performs \rd{}, we replace it with a call to \rd($ts$).
Finally, we return the result of the modified sequential algorithm.
We linearized $Q$ at the point the \snapshot{} was taken.

Using this transformation, we can prove the following theorem.

\begin{theorem}
  Given any query operation $Q$ that is computable on a regular, external BST, we can add $Q$ as a linearizable operation to the \NBBST{} after some modifications.
  These modifications preserve the runtime bounds of the original \NBBST{} operations.
\end{theorem}

\begin{theorem}
  A non-blocking BST can support \ins{}, \del{}, \find{}, and \pred{} in $O(h + c)$ amortized time where $h$ is the height of the tree at the start of the operation and $c$ is the number of operations concurrent with the current operation. \Hao{the bounds for $c$ can be improved, but I'm stating it this way for simplicity.}
\end{theorem}

\section{Chromatic Tree Example}



\subsection{Snapshot object}

How would the current value of the object be defined?
